Logarithmic scaling of higher-order temperature moments in the atmospheric surface layer

A generalized logarithmic law for high-order moments of passive scalars is proposed for turbulent boundary layers. This law is analogous to the generalized log law that has been proposed for high-order moments of the turbulent longitudinal velocity and is derived by combining the random sweeping decorrelation hypothesis with a spectral model informed by the attached eddy hypothesis. The proposed theory predicts that the high-order moments of passive scalar fluctuations within the inertial sublayer will vary logarithmically with wall-normal distance ($z$). The proposed theory is evaluated using high frequency time-series measurements of temperature and streamwise velocity fluctuations obtained in the first meter of the atmospheric surface layer (ASL) under near-neutral thermal stratification. The logarithmic dependence with $z$ within the inertial sublayer is observed in both the air temperature and velocity moments, with good agreement to the predictions from the proposed theory. Surprisingly, the proposed theory appears to be as, if not more, valid for transported passive scalars than for the longitudinal velocity.

==> figures/fig files/dist_diff2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.99216,0.55294,0.23529}%
\definecolor{mycolor2}{rgb}{0.25882,0.57255,0.77647}%
\definecolor{mycolor3}{rgb}{0.85098,0.28235,0.00392}%
\definecolor{mycolor4}{rgb}{0.14510,0.38039,0.59804}%
\definecolor{mycolor5}{rgb}{0.65098,0.21176,0.01176}%
\definecolor{mycolor6}{rgb}{0.08824,0.28431,0.50882}%
\definecolor{mycolor7}{rgb}{0.49804,0.15294,0.01569}%
\definecolor{mycolor8}{rgb}{0.03137,0.18824,0.41961}%
%
\newcommand\Height{1.1in}
\newcommand\Width{1.5in}
\newcommand\VSKIP{1.35in}

\begin{tikzpicture}


\begin{axis}[%
width=\Width,
height=\Height,
at={(.0in,\VSKIP*3)},
scale only axis,
xmin=-5.5,
xmax=5.5,
xlabel style={font=\color{white!15!black}},%xlabel={$\text{u'/}\sigma{}_\text{u}\text{    ,  }\theta'\sigma{}_\theta$},
ymode=log,
ymin=0.25,
ymax=64, % ymin=0.909090909,% ymax=1.1,
ytick={0.0625, 0.125, 0.25, 0.5, 1, 2, 4, 8, 16, 32, 64}, 
yticklabels={$1/16$, $1/8$, $1/4$, $1/2$ ,$1$, $2$ ,$4$,$8$ , $16$, $32$ , $64$},
xtick={-5,-4,-3,-2,-1,0,1,2,3,4,5}, 
xticklabels={-5,-4,-3,-2,-1,0,1,2,3,4,5},
ticklabel style = {font=\footnotesize} ,
yminorticks=true,
ylabel style={font=\color{white!15!black}, text width=2.5cm},
ylabel= {$\mathrm{PDF}_{exp}/\mathrm{PDF}_{norm}$},% ylabel= {$\mathrm{pdf(u'/\sigma_{u})}_{exp}/\mathrm{pdf}_{norm}$ \\ $\mathrm{pdf(\theta'/\sigma_{\theta})}_{exp}/\mathrm{pdf}_{norm}$},
axis background/.style={fill=white},
ylabel shift = -4pt,
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(1.,0.03)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black,draw=none}
]
\node[fill = white, rotate =0, anchor = center] (z1) at (axis cs:0,32) {$z = 1.0$ m};

\addplot [color=mycolor2, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor2}]
  table[row sep=crcr]{%
-4.39069521075637	4.8664206884064\\
-4.34306742444763	2.23796013392579\\
-4.2954396381389	0.88414609918375\\
-4.24781185183017	0.682802849834665\\
-4.20018406552144	0.985825116602566\\
-4.1525562792127	1.70785995751355\\
-4.10492849290397	2.35975189656657\\
-4.05730070659524	1.75125388156099\\
-4.00967292028651	1.88728759521962\\
-3.96204513397778	1.59675586733237\\
-3.91441734766904	1.58065524208255\\
-3.86678956136031	2.10770399091219\\
-3.81916177505158	1.57346217397241\\
-3.77153398874285	1.3912913168666\\
-3.72390620243411	1.63004688846648\\
-3.67627841612538	1.97060006254852\\
-3.62865062981665	1.92877546813837\\
-3.58102284350792	1.82409359721261\\
-3.53339505719918	2.10910738975679\\
-3.48576727089045	2.10868474916597\\
-3.43813948458172	1.83288724531802\\
-3.39051169827299	1.71543937413641\\
-3.34288391196426	1.82742017360357\\
-3.29525612565552	2.0150805140029\\
-3.24762833934679	1.88521319323863\\
-3.20000055303806	1.89201152631668\\
-3.15237276672933	1.77971021964523\\
-3.10474498042059	1.69815767028111\\
-3.05711719411186	1.70182613466115\\
-3.00948940780313	1.63073878848081\\
-2.9618616214944	1.65105518360809\\
-2.91423383518567	1.60043806369384\\
-2.86660604887693	1.49265904925476\\
-2.8189782625682	1.47192630521524\\
-2.77135047625947	1.45070884775941\\
-2.72372268995074	1.49016253262184\\
-2.676094903642	1.45733484687755\\
-2.62846711733327	1.4019517566533\\
-2.58083933102454	1.42277724703369\\
-2.53321154471581	1.43663230856148\\
-2.48558375840708	1.40348187569856\\
-2.43795597209834	1.33839778513063\\
-2.39032818578961	1.29428076992368\\
-2.34270039948088	1.34020441168614\\
-2.29507261317215	1.30120928054437\\
-2.24744482686341	1.27034095982241\\
-2.19981704055468	1.2666284661266\\
-2.15218925424595	1.20436924582335\\
-2.10456146793722	1.20632481178065\\
-2.05693368162849	1.22308788984565\\
-2.00930589531975	1.19686474151918\\
-1.96167810901102	1.17247816993728\\
-1.91405032270229	1.17973288156322\\
-1.86642253639356	1.15892726831669\\
-1.81879475008482	1.14075298795122\\
-1.77116696377609	1.16182973697378\\
-1.72353917746736	1.12727849662786\\
-1.67591139115863	1.11686149094863\\
-1.6282836048499	1.12625210951105\\
-1.58065581854116	1.12160656859833\\
-1.53302803223243	1.13137825794116\\
-1.4854002459237	1.14002537596242\\
-1.43777245961497	1.12355348608651\\
-1.39014467330623	1.11747302021018\\
-1.3425168869975	1.10544016357058\\
-1.29488910068877	1.09789957713625\\
-1.24726131438004	1.10143092808223\\
-1.19963352807131	1.08316108345666\\
-1.15200574176257	1.0680374677614\\
-1.10437795545384	1.07715971081277\\
-1.05675016914511	1.07597267811781\\
-1.00912238283638	1.06812475579533\\
-0.961494596527644	1.05549348168776\\
-0.913866810218912	1.05440799391098\\
-0.86623902391018	1.03099849689054\\
-0.818611237601447	1.0150319758816\\
-0.770983451292715	1.02452294200079\\
-0.723355664983983	1.02313267788602\\
-0.675727878675251	1.01192792934462\\
-0.628100092366518	1.0019064677352\\
-0.580472306057786	0.989524266403789\\
-0.532844519749054	0.981217163681299\\
-0.485216733440322	0.966551329880123\\
-0.437588947131589	0.95534126798881\\
-0.389961160822857	0.94749042687904\\
-0.342333374514125	0.949954499735291\\
-0.294705588205393	0.938088345654765\\
-0.247077801896661	0.921620126442921\\
-0.199450015587928	0.918035885590359\\
-0.151822229279196	0.918144875663875\\
-0.104194442970464	0.908659221240788\\
-0.0565666566617314	0.90643641060278\\
-0.0089388703529994	0.900692668092461\\
0.038688915955733	0.89371630122978\\
0.086316702264465	0.890123982671986\\
0.133944488573197	0.891950570407484\\
0.181572274881929	0.894014124405725\\
0.229200061190661	0.890458172704423\\
0.276827847499394	0.8923541490089\\
0.324455633808126	0.89622165408508\\
0.372083420116858	0.898941431132458\\
0.419711206425591	0.897731079829443\\
0.467338992734323	0.890387090508208\\
0.514966779043055	0.892617855465641\\
0.562594565351787	0.898208713325151\\
0.61022235166052	0.896120864568687\\
0.657850137969252	0.903736223252961\\
0.705477924277984	0.915696615383502\\
0.753105710586716	0.920234562220772\\
0.800733496895449	0.925801362537666\\
0.848361283204181	0.931730210629279\\
0.895989069512913	0.94129926260348\\
0.943616855821646	0.945395164816108\\
0.991244642130378	0.961143544415915\\
1.03887242843911	0.977757285427128\\
1.08650021474784	0.977530701202659\\
1.13412800105657	0.971371373105809\\
1.18175578736531	0.99666179885979\\
1.22938357367404	1.0141491455427\\
1.27701135998277	1.02071788199931\\
1.3246391462915	1.0150575195351\\
1.37226693260024	1.02122550649487\\
1.41989471890897	1.05177486053015\\
1.4675225052177	1.08451710803855\\
1.51515029152643	1.09990588591286\\
1.56277807783516	1.1173598594158\\
1.6104058641439	1.12235378816136\\
1.65803365045263	1.12067132754646\\
1.70566143676136	1.15318438645829\\
1.75328922307009	1.16016898387862\\
1.80091700937883	1.18945570713626\\
1.84854479568756	1.24239967350391\\
1.89617258199629	1.27064602754014\\
1.94380036830502	1.29632813274509\\
1.99142815461375	1.32558239960043\\
2.03905594092249	1.3492420466971\\
2.08668372723122	1.38493110352474\\
2.13431151353995	1.45202878477453\\
2.18193929984868	1.44764278473031\\
2.22956708615742	1.47816981883359\\
2.27719487246615	1.51226102235748\\
2.32482265877488	1.54351211047798\\
2.37245044508361	1.61784860088147\\
2.42007823139235	1.71185575900779\\
2.46770601770108	1.78511768785488\\
2.51533380400981	1.81157624174853\\
2.56296159031854	1.85201232972524\\
2.61058937662727	1.84789942532131\\
2.65821716293601	1.99504433853614\\
2.70584494924474	1.97598746873146\\
2.75347273555347	2.08123315262082\\
2.8011005218622	2.23000586404703\\
2.84872830817093	2.26576519618384\\
2.89635609447967	2.38558657752122\\
2.9439838807884	2.60523966821174\\
2.99161166709713	2.77538996634897\\
3.03923945340586	2.65119661575113\\
3.0868672397146	2.56845404206886\\
3.13449502602333	2.90992647104435\\
3.18212281233206	3.30971527288641\\
3.22975059864079	3.47733777238359\\
3.27737838494953	3.36586432700056\\
3.32500617125826	3.53869364953475\\
3.37263395756699	3.9983885741044\\
3.42026174387572	4.24845038406425\\
3.46788953018445	4.2391378628796\\
3.51551731649319	4.60896817627702\\
3.56314510280192	4.82846590338005\\
3.61077288911065	4.6483395620138\\
3.65840067541938	4.93024152553921\\
3.70602846172812	5.57740537218249\\
3.75365624803685	5.52298693496769\\
3.80128403434558	5.11857484090036\\
3.84891182065431	5.71764487726564\\
3.89653960696304	5.99918243011348\\
3.94416739327178	6.04177267181511\\
3.99179517958051	5.96409388418776\\
4.03942296588924	6.6395953377271\\
4.08705075219797	8.4967181732616\\
4.13467853850671	9.52200558444528\\
4.18230632481544	8.66395196037067\\
4.22993411112417	7.31250502593733\\
4.2775618974329	10.2058720597761\\
4.32518968374163	8.37687655437026\\
4.37281747005037	10.3644968144254\\
4.4204452563591	12.325025273382\\
4.46807304266783	17.9769749290983\\
4.51570082897656	11.3342113760262\\
4.56332861528529	8.41567499121726\\
4.61095640159403	9.2122266601358\\
4.65858418790276	4.40170315840666\\
4.70621197421149	12.6480063633441\\
4.75383976052022	18.1576733217085\\
4.80146754682896	19.307091261041\\
4.84909533313769	9.82415377791285\\
4.89672311944642	1.53163326057062\\
4.94435090575515	0\\
4.99197869206389	0\\
5.03960647837262	20.3385527872252\\
5.08723426468135	97.8448396556348\\
};
\addlegendentry{$\text{u'/}\sigma{}_\text{u}$}

\addplot [color=mycolor1, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-4.65891264028589	15.6493637185169\\
-4.61176778719693	4.52608763180296\\
-4.56462293410797	6.15597520025579\\
-4.51747808101902	5.76217006972365\\
-4.47033322793006	4.93294180198555\\
-4.42318837484111	12.3156531387154\\
-4.37604352175215	7.48807852395771\\
-4.3288986686632	5.83053608635242\\
-4.28175381557424	5.51985646543939\\
-4.23460896248528	5.98960855705225\\
-4.18746410939633	6.20486486635459\\
-4.14031925630737	6.79639389627035\\
-4.09317440321842	6.66748471909114\\
-4.04602955012946	4.84572294354371\\
-3.99888469704051	3.62329992805698\\
-3.95173984395155	5.08937568793846\\
-3.9045949908626	5.89700585781599\\
-3.85745013777364	5.61590968929254\\
-3.81030528468468	4.80490829928088\\
-3.76316043159573	4.70272614751019\\
-3.71601557850677	5.41347613068532\\
-3.66887072541782	4.60793473674264\\
-3.62172587232886	4.96855722094634\\
-3.57458101923991	5.25527908715587\\
-3.52743616615095	4.7960528837042\\
-3.480291313062	4.64799639168047\\
-3.43314645997304	4.68661963823481\\
-3.38600160688408	4.31027218991714\\
-3.33885675379513	3.95410649711853\\
-3.29171190070617	3.87712834093609\\
-3.24456704761722	3.69061500438663\\
-3.19742219452826	3.32851838255591\\
-3.15027734143931	3.47254530632254\\
-3.10313248835035	3.36790928093801\\
-3.05598763526139	3.34060879590417\\
-3.00884278217244	3.39749711690195\\
-2.96169792908348	2.96875378275355\\
-2.91455307599453	3.02064376861609\\
-2.86740822290557	2.78105170117853\\
-2.82026336981662	2.61051741894824\\
-2.77311851672766	2.7702385014077\\
-2.72597366363871	2.69915936251575\\
-2.67882881054975	2.64725594833568\\
-2.63168395746079	2.63508279909224\\
-2.58453910437184	2.54563408477132\\
-2.53739425128288	2.46009921223917\\
-2.49024939819393	2.32775537550988\\
-2.44310454510497	2.23239092811152\\
-2.39595969201602	2.23389622830254\\
-2.34881483892706	2.14373481729905\\
-2.3016699858381	2.11179226095421\\
-2.25452513274915	2.05066287436208\\
-2.20738027966019	1.97000292531143\\
-2.16023542657124	1.90324392821774\\
-2.11309057348228	1.87823820920728\\
-2.06594572039333	1.82681940656791\\
-2.01880086730437	1.76266535283199\\
-1.97165601421542	1.7292879810705\\
-1.92451116112646	1.66308927189958\\
-1.8773663080375	1.6030398461525\\
-1.83022145494855	1.56679481790019\\
-1.78307660185959	1.54137403273257\\
-1.73593174877064	1.49638800723781\\
-1.68878689568168	1.44355097832683\\
-1.64164204259273	1.39658089269466\\
-1.59449718950377	1.33692623606906\\
-1.54735233641482	1.31173354288463\\
-1.50020748332586	1.27339287161864\\
-1.4530626302369	1.24015089243381\\
-1.40591777714795	1.2024375472035\\
-1.35877292405899	1.1560625795384\\
-1.31162807097004	1.12558524904768\\
-1.26448321788108	1.12159390607524\\
-1.21733836479213	1.08321895724439\\
-1.17019351170317	1.06416552356826\\
-1.12304865861421	1.02918075129672\\
-1.07590380552526	1.01113199010916\\
-1.0287589524363	0.993144282727369\\
-0.981614099347348	0.980269298210478\\
-0.934469246258392	0.959826393944399\\
-0.887324393169437	0.952936021496826\\
-0.840179540080481	0.943689811799999\\
-0.793034686991525	0.935709396558863\\
-0.74588983390257	0.916014314430531\\
-0.698744980813614	0.897706173365232\\
-0.651600127724659	0.901558056514313\\
-0.604455274635703	0.896283246307555\\
-0.557310421546747	0.885070089024194\\
-0.510165568457792	0.877402687059909\\
-0.463020715368836	0.876340627201606\\
-0.415875862279881	0.881178061704802\\
-0.368731009190925	0.88574074927123\\
-0.321586156101969	0.875493530770296\\
-0.274441303013014	0.875199658010558\\
-0.227296449924058	0.868287531660324\\
-0.180151596835102	0.871508267840501\\
-0.133006743746147	0.868950889512225\\
-0.0858618906571912	0.862025445489704\\
-0.0387170375682358	0.868523638098454\\
0.00842781552072008	0.871138882815561\\
0.0555726686096756	0.872827276809879\\
0.102717521698631	0.870537093019286\\
0.149862374787587	0.877695518833032\\
0.197007227876543	0.885454270341804\\
0.244152080965498	0.879158118046363\\
0.291296934054454	0.890336737870403\\
0.338441787143409	0.88429700732066\\
0.385586640232365	0.89418318587943\\
0.432731493321321	0.903936552924624\\
0.479876346410276	0.910438277816075\\
0.527021199499232	0.919619676697098\\
0.574166052588188	0.934949431483268\\
0.621310905677143	0.942848106904353\\
0.668455758766099	0.953283698699044\\
0.715600611855054	0.94937047973822\\
0.76274546494401	0.942939292538229\\
0.809890318032966	0.955126857749635\\
0.857035171121921	0.971441300626737\\
0.904180024210877	0.982812595390276\\
0.951324877299832	1.00166533630786\\
0.998469730388788	1.0093090006131\\
1.04561458347774	1.01120056817746\\
1.0927594365667	1.01909677282499\\
1.13990428965565	1.0372566915418\\
1.18704914274461	1.04726641910784\\
1.23419399583357	1.04142116256359\\
1.28133884892252	1.0644079007036\\
1.32848370201148	1.10096367447684\\
1.37562855510043	1.11082513122083\\
1.42277340818939	1.11651420530381\\
1.46991826127834	1.13631917643581\\
1.5170631143673	1.14558173977093\\
1.56420796745626	1.1784765099052\\
1.61135282054521	1.18931312514035\\
1.65849767363417	1.18508824027509\\
1.70564252672312	1.21181631578746\\
1.75278737981208	1.23268587260112\\
1.79993223290103	1.2560431418093\\
1.84707708598999	1.28808453832409\\
1.89422193907894	1.27596205211733\\
1.9413667921679	1.29384704399476\\
1.98851164525686	1.32963694496835\\
2.03565649834581	1.37856421104478\\
2.08280135143477	1.3895341716084\\
2.12994620452372	1.41354713205848\\
2.17709105761268	1.45944380884683\\
2.22423591070163	1.46483539807387\\
2.27138076379059	1.45243894807265\\
2.31852561687954	1.5130037873836\\
2.3656704699685	1.51205866671463\\
2.41281532305746	1.5709087423252\\
2.45996017614641	1.60705224972303\\
2.50710502923537	1.69448614960026\\
2.55424988232432	1.74401853019693\\
2.60139473541328	1.83641287305376\\
2.64853958850223	1.91356668872837\\
2.69568444159119	1.9713619030993\\
2.74282929468015	2.0261208551739\\
2.7899741477691	2.06566316256956\\
2.83711900085806	2.18788520025677\\
2.88426385394701	2.25501230204998\\
2.93140870703597	2.33641752777333\\
2.97855356012492	2.5734686091309\\
3.02569841321388	2.48108468681031\\
3.07284326630283	2.51172413528935\\
3.11998811939179	2.78499026004779\\
3.16713297248075	2.86488673591969\\
3.2142778255697	2.97394697651467\\
3.26142267865866	3.20904272795035\\
3.30856753174761	3.15724625204996\\
3.35571238483657	3.21351796554514\\
3.40285723792552	3.29910143445587\\
3.45000209101448	3.31296571411201\\
3.49714694410344	3.47820014180935\\
3.54429179719239	3.89358278547087\\
3.59143665028135	4.85228341894763\\
3.6385815033703	5.06929008910668\\
3.68572635645926	4.63848472504926\\
3.73287120954821	5.31714635080568\\
3.78001606263717	5.29474352950143\\
3.82716091572612	5.41384276298549\\
3.87430576881508	5.62363480227984\\
3.92145062190404	4.69319276314299\\
3.96859547499299	5.19707910181433\\
4.01574032808195	6.57696529469461\\
4.0628851811709	7.21960471527531\\
4.11003003425986	6.51685423833685\\
4.15717488734881	8.21126478700659\\
4.20431974043777	9.48170459937625\\
4.25146459352673	8.86968914577587\\
4.29860944661568	7.47793755144391\\
4.34575429970464	10.6801956568971\\
4.39289915279359	13.2640371520861\\
4.44004400588255	11.6087800121257\\
4.4871888589715	12.4347171991675\\
4.53433371206046	20.4791293835261\\
4.58147856514941	18.192853210662\\
4.62862341823837	11.6144957872029\\
4.67576827132733	12.630854684133\\
4.72291312441628	27.8440702464942\\
};
\addlegendentry{$\theta\text{'/}\sigma{}_\theta$}


\addplot [color=black, dashed, line width = 0.5pt]
  table[row sep=crcr]{%
-6	1\\
6	1\\
};
\addlegendentry{\footnotesize Gaussian};

% \addplot[area legend, draw=black, fill=black, fill opacity=0.01]
% table[row sep=crcr] {%
% x	y\\
% -6	0.909090909090\\
% 6	0.909090909090\\
% 6	1.1\\
% -6	1.1\\
% }--cycle;
 \addplot[fill=black, fill opacity = 0.1, draw = none,area legend] coordinates {(-6,0.9090909090) (6,0.9090909090) (6,1.1) (-6,1.1)};
\addlegendentry{\footnotesize $\pm10\%$};

\end{axis}

\begin{axis}[%
width=\Width,
height=\Height,
at={(0in,\VSKIP*2)},
scale only axis,
xmin=-5.5,
xmax=5.5,
xlabel style={font=\color{white!15!black}},%xlabel={$\text{u'/}\sigma{}_\text{u}\text{    ,  }\theta\text{'/}\sigma{}_\theta$},
ymode=log,
ymin=0.25,
ymax=64, % ymin=0.909090909,% ymax=1.1,
ytick={0.0625, 0.125, 0.25, 0.5, 1, 2, 4, 8, 16, 32, 64}, 
yticklabels={$1/16$, $1/8$, $1/4$, $1/2$ ,$1$, $2$ ,$4$,$8$ , $16$, $32$ , $64$},
xtick={-5,-4,-3,-2,-1,0,1,2,3,4,5}, 
xticklabels={-5,-4,-3,-2,-1,0,1,2,3,4,5},
ticklabel style = {font=\footnotesize} ,
yminorticks=true,
ylabel style={font=\color{white!15!black}, text width=2.5cm},
ylabel= {$\mathrm{PDF}_{exp}/\mathrm{PDF}_{norm}$},% ylabel= {$\mathrm{pdf(u'/\sigma_{u})}_{exp}/\mathrm{pdf}_{norm}$ \\ $\mathrm{pdf(\theta'/\sigma_{\theta})}_{exp}/\mathrm{pdf}_{norm}$},
axis background/.style={fill=white},
ylabel shift = -4pt,
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(1.,0.03)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black,draw=none}
]

\node[fill = white, rotate =0, anchor = center] (z1) at (axis cs:0,32) {$z = 0.25$ m};

\addplot [color=mycolor4, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor4}]
  table[row sep=crcr]{%
-4.04518965615418	1.33899683810615\\
-3.99746426648285	0.54744865154561\\
-3.94973887681151	0.169579207049623\\
-3.90201348714018	0.454508802665379\\
-3.85428809746885	0.463206280777494\\
-3.80656270779752	0.595919169161514\\
-3.75883731812618	0.43173342844369\\
-3.71111192845485	0.478725088329991\\
-3.66338653878352	0.626331726608728\\
-3.61566114911218	0.971153801546105\\
-3.56793575944085	0.854148819908763\\
-3.52021036976952	0.631780664910649\\
-3.47248498009818	0.58067450186139\\
-3.42475959042685	0.744308408207667\\
-3.37703420075552	0.680408426704196\\
-3.32930881108419	0.647606231464743\\
-3.28158342141285	0.675353873184975\\
-3.23385803174152	0.657514892520329\\
-3.18613264207019	0.733791899437038\\
-3.13840725239885	0.778644692873976\\
-3.09068186272752	0.759052021367531\\
-3.04295647305619	0.72112529655722\\
-2.99523108338485	0.619432292312034\\
-2.94750569371352	0.636910347734444\\
-2.89978030404219	0.682982134128949\\
-2.85205491437086	0.687353977326754\\
-2.80432952469952	0.713210534434708\\
-2.75660413502819	0.690786460025102\\
-2.70887874535686	0.749266285776037\\
-2.66115335568552	0.730896177196551\\
-2.61342796601419	0.776006440462986\\
-2.56570257634286	0.785455698568893\\
-2.51797718667152	0.822891948268602\\
-2.47025179700019	0.82228893895618\\
-2.42252640732886	0.855457927193357\\
-2.37480101765752	0.837043174903278\\
-2.32707562798619	0.847408271780533\\
-2.27935023831486	0.864736510723334\\
-2.23162484864353	0.847817787411317\\
-2.18389945897219	0.852256233097154\\
-2.13617406930086	0.894095027199099\\
-2.08844867962953	0.931115962051764\\
-2.04072328995819	0.968980581164496\\
-1.99299790028686	0.945057837812232\\
-1.94527251061553	0.940837415243576\\
-1.89754712094419	0.963451440452263\\
-1.84982173127286	0.966917351361614\\
-1.80209634160153	0.998860627217255\\
-1.7543709519302	0.98869893467253\\
-1.70664556225886	0.992118642926732\\
-1.65892017258753	0.991780462695351\\
-1.6111947829162	1.01693637986527\\
-1.56346939324486	1.04034823688266\\
-1.51574400357353	1.02915507525699\\
-1.4680186139022	1.02346763536452\\
-1.42029322423086	1.0403680291578\\
-1.37256783455953	1.04623065899861\\
-1.3248424448882	1.04342487422116\\
-1.27711705521686	1.05737073729508\\
-1.22939166554553	1.06269225370322\\
-1.1816662758742	1.04844227035766\\
-1.13394088620287	1.04909563755324\\
-1.08621549653153	1.04749007181562\\
-1.0384901068602	1.04388132165809\\
-0.990764717188867	1.04940581167364\\
-0.943039327517534	1.04256475084395\\
-0.895313937846201	1.04675541121491\\
-0.847588548174868	1.04321253479308\\
-0.799863158503535	1.04552412442363\\
-0.752137768832201	1.04999702491747\\
-0.704412379160869	1.05655222273774\\
-0.656686989489535	1.05188006522465\\
-0.608961599818203	1.04574087865482\\
-0.561236210146869	1.04260021113627\\
-0.513510820475536	1.04334975451777\\
-0.465785430804203	1.04464372654196\\
-0.41806004113287	1.03963913323206\\
-0.370334651461537	1.039262862526\\
-0.322609261790204	1.02780265173094\\
-0.274883872118871	1.01740986103756\\
-0.227158482447538	1.01960409310366\\
-0.179433092776205	1.0299802385078\\
-0.131707703104872	1.02514130307975\\
-0.0839823134335389	1.01168750679978\\
-0.0362569237622061	1.00049551495692\\
0.0114684659091272	1.00379620853047\\
0.0591938555804602	0.992171718081978\\
0.106919245251793	0.99345659087955\\
0.154644634923126	0.993136882135712\\
0.202370024594459	0.99543761100079\\
0.250095414265792	0.993065978492403\\
0.297820803937125	0.975638981989618\\
0.345546193608458	0.979467612436256\\
0.393271583279792	0.969245668410569\\
0.440996972951125	0.969594593567776\\
0.488722362622458	0.964702380312142\\
0.536447752293791	0.969554873208208\\
0.584173141965124	0.96059426561864\\
0.631898531636457	0.958749922326045\\
0.67962392130779	0.957423248465045\\
0.727349310979123	0.948472348257524\\
0.775074700650456	0.940095264335015\\
0.822800090321789	0.94374444072323\\
0.870525479993122	0.944774579093508\\
0.918250869664455	0.936916683291806\\
0.965976259335788	0.931976775433008\\
1.01370164900712	0.933549443685117\\
1.06142703867845	0.928683285551091\\
1.10915242834979	0.922143746921177\\
1.15687781802112	0.927786620849644\\
1.20460320769245	0.926598728790848\\
1.25232859736379	0.914506804773131\\
1.30005398703512	0.921825202624152\\
1.34777937670645	0.937893665156176\\
1.39550476637779	0.939483162492325\\
1.44323015604912	0.936008227208557\\
1.49095554572045	0.940263005480199\\
1.53868093539178	0.954807667767239\\
1.58640632506312	0.968994202593298\\
1.63413171473445	0.956890284126314\\
1.68185710440578	0.92623678381433\\
1.72958249407712	0.953129170785173\\
1.77730788374845	0.988692561929129\\
1.82503327341978	0.997935703170742\\
1.87275866309112	1.00120231325523\\
1.92048405276245	1.00316069551315\\
1.96820944243378	1.02483111181154\\
2.01593483210511	1.02415339342809\\
2.06366022177645	1.02184655933824\\
2.11138561144778	1.04694004854736\\
2.15911100111911	1.08584754652249\\
2.20683639079045	1.08584550564329\\
2.25456178046178	1.09384688942108\\
2.30228717013311	1.11019563115321\\
2.35001255980445	1.12872156355654\\
2.39773794947578	1.14889877397515\\
2.44546333914711	1.20204924099089\\
2.49318872881845	1.24226330976417\\
2.54091411848978	1.29216239315096\\
2.58863950816111	1.2752842362405\\
2.63636489783244	1.35294123411359\\
2.68409028750378	1.45921853817683\\
2.73181567717511	1.39547813710458\\
2.77954106684644	1.49810149033925\\
2.82726645651778	1.62460647316422\\
2.87499184618911	1.61713941037295\\
2.92271723586044	1.74646664939997\\
2.97044262553178	1.82046916657645\\
3.01816801520311	1.97204876073059\\
3.06589340487444	2.01943452543922\\
3.11361879454577	2.03526634726849\\
3.16134418421711	2.10154558107758\\
3.20906957388844	2.20235671154665\\
3.25679496355977	2.34117150213211\\
3.30452035323111	2.4170547255994\\
3.35224574290244	2.56320003181532\\
3.39997113257377	2.64651822614021\\
3.44769652224511	3.05148947819652\\
3.49542191191644	3.30525976955377\\
3.54314730158777	3.2801623836428\\
3.5908726912591	3.96880340514527\\
3.63859808093044	3.79813922575274\\
3.68632347060177	3.93670336312359\\
3.7340488602731	3.49005741727553\\
3.78177424994444	4.07582475849087\\
3.82949963961577	4.43234154999775\\
3.8772250292871	5.28543303644628\\
3.92495041895844	5.88917608554547\\
3.97267580862977	6.00753863423161\\
4.0204011983011	6.38859170629829\\
4.06812658797244	7.36926751423228\\
4.11585197764377	5.18724635303876\\
4.1635773673151	6.82214288333404\\
4.21130275698643	8.74661439857402\\
4.25902814665777	10.6218260008029\\
4.3067535363291	8.12529943465146\\
4.35447892600043	9.08880935424959\\
4.40220431567177	13.0324641104986\\
4.4499297053431	15.6938723209118\\
4.49765509501443	12.4005552700241\\
4.54538048468577	13.9582075268564\\
4.5931058743571	17.539508894259\\
4.64083126402843	19.6953719493523\\
4.68855665369977	34.6263480415164\\
4.7362820433711	22.8581534430249\\
4.78400743304243	9.64723549465872\\
4.83173282271376	10.5069431462649\\
4.8794582123851	22.6598658075827\\
4.92718360205643	36.9743407944086\\
4.97490899172776	44.7480553395137\\
5.0226343813991	64.6728993114211\\
5.07035977107043	20.6910527181257\\
5.11808516074176	31.761020971945\\
5.1658105504131	56.3762152620354\\
5.21353594008443	98.7493884877112\\
5.26126132975576	85.9246752088672\\
5.30898671942709	77.153773734947\\
5.35671210909843	16.1158255973481\\
5.40443749876976	138.408108185943\\
5.45216288844109	665.85461090425\\
};
\addlegendentry{$\text{u'/}\sigma{}_\text{u}$}

\addplot [color=mycolor3, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor3}]
  table[row sep=crcr]{%
-4.02029280022338	1.24150484063745\\
-3.97687440003228	0.350335387428369\\
-3.93345599984118	0.447367403775875\\
-3.89003759965008	0.488360252268205\\
-3.84661919945897	0.458336900731874\\
-3.80320079926787	0.278204290599367\\
-3.75978239907677	0.344229525206817\\
-3.71636399888566	0.629811546362177\\
-3.67294559869456	0.632448667771804\\
-3.62952719850346	0.615333436209809\\
-3.58610879831235	0.546385287682137\\
-3.54269039812125	0.492625261744652\\
-3.49927199793015	0.545744538707776\\
-3.45585359773905	0.648234453018204\\
-3.41243519754794	0.792438606579526\\
-3.36901679735684	0.810220711338479\\
-3.32559839716574	0.853982595493025\\
-3.28217999697463	0.869722001700905\\
-3.23876159678353	0.862122104015613\\
-3.19534319659243	0.86724824040893\\
-3.15192479640132	0.915540588143672\\
-3.10850639621022	0.939827197445304\\
-3.06508799601912	0.987040522647391\\
-3.02166959582801	1.03116837983026\\
-2.97825119563691	1.02681281315443\\
-2.93483279544581	1.02422028303056\\
-2.89141439525471	1.12218339579472\\
-2.8479959950636	1.21153286109154\\
-2.8045775948725	1.11994892854621\\
-2.7611591946814	1.11230311803407\\
-2.71774079449029	1.14133831155519\\
-2.67432239429919	1.14610750618597\\
-2.63090399410809	1.13561185085062\\
-2.58748559391698	1.10880210291028\\
-2.54406719372588	1.1076537023042\\
-2.50064879353478	1.13424039715147\\
-2.45723039334367	1.12098904422696\\
-2.41381199315257	1.06198020357742\\
-2.37039359296147	1.11252550184996\\
-2.32697519277037	1.10587860191171\\
-2.28355679257926	1.14751297371026\\
-2.24013839238816	1.13200601814129\\
-2.19671999219706	1.09734202672404\\
-2.15330159200595	1.08877024108604\\
-2.10988319181485	1.09843900378273\\
-2.06646479162375	1.08358641755863\\
-2.02304639143264	1.09287220431508\\
-1.97962799124154	1.09476548079612\\
-1.93620959105044	1.11766383660004\\
-1.89279119085933	1.11329016185389\\
-1.84937279066823	1.07965263107604\\
-1.80595439047713	1.06201580641781\\
-1.76253599028603	1.06802258039507\\
-1.71911759009492	1.07441714990311\\
-1.67569918990382	1.07352684085775\\
-1.63228078971272	1.07307822090976\\
-1.58886238952161	1.06285704434639\\
-1.54544398933051	1.04986301114837\\
-1.50202558913941	1.04661556252603\\
-1.4586071889483	1.04405790091044\\
-1.4151887887572	1.0322827438719\\
-1.3717703885661	1.03193531795562\\
-1.328351988375	1.03006153822267\\
-1.28493358818389	1.03210108965689\\
-1.24151518799279	1.0254706876566\\
-1.19809678780169	1.02779997109685\\
-1.15467838761058	1.02050844910799\\
-1.11125998741948	1.00400179530824\\
-1.06784158722838	0.993701810522813\\
-1.02442318703727	1.00517052588074\\
-0.98100478684617	1.00517891437214\\
-0.937586386655067	1.00419404314221\\
-0.894167986463964	0.999847999304847\\
-0.850749586272861	1.00586552572845\\
-0.807331186081758	1.0086130946513\\
-0.763912785890655	0.993903016834918\\
-0.720494385699552	0.986403379360377\\
-0.677075985508449	0.986354614027381\\
-0.633657585317346	0.985361043746002\\
-0.590239185126243	0.97997598399714\\
-0.54682078493514	0.983546373133303\\
-0.503402384744037	0.970306602598333\\
-0.459983984552933	0.967471059746723\\
-0.41656558436183	0.981990591326556\\
-0.373147184170727	0.989577765154901\\
-0.329728783979624	0.974611652728294\\
-0.286310383788521	0.966903414726825\\
-0.242891983597418	0.984102646252472\\
-0.199473583406315	0.986818186864795\\
-0.156055183215212	0.971607062308246\\
-0.112636783024109	0.972267266425847\\
-0.0692183828330057	0.963245881399919\\
-0.0257999826419024	0.96974491526712\\
0.0176184175492003	0.973221693828618\\
0.0610368177403033	0.964905733568174\\
0.104455217931407	0.965938052677435\\
0.14787361812251	0.960847305431317\\
0.191292018313613	0.965951647590317\\
0.234710418504716	0.97021987526091\\
0.278128818695819	0.964177054012828\\
0.321547218886922	0.964397484533543\\
0.364965619078025	0.969139606993595\\
0.408384019269128	0.976303755059496\\
0.451802419460231	0.98568111198234\\
0.495220819651334	0.985663865823847\\
0.538639219842437	0.985071950688628\\
0.582057620033541	0.981682079968776\\
0.625476020224643	0.972164496701877\\
0.668894420415746	0.975194454873839\\
0.71231282060685	0.974578250112613\\
0.755731220797953	0.96987806547078\\
0.799149620989056	0.972710020592657\\
0.842568021180159	0.972307010768925\\
0.885986421371262	0.983610720959341\\
0.929404821562365	0.98827183727488\\
0.972823221753468	0.98322245112372\\
1.01624162194457	0.992311929372483\\
1.05966002213567	0.995889674110928\\
1.10307842232678	0.994877974340514\\
1.14649682251788	0.988357619070194\\
1.18991522270898	0.991037714511377\\
1.23333362290009	0.996396745258182\\
1.27675202309119	0.994610268013095\\
1.32017042328229	1.00001106339331\\
1.3635888234734	0.998048518094718\\
1.4070072236645	1.00589418133046\\
1.4504256238556	1.00380024365538\\
1.49384402404671	1.01879827367433\\
1.53726242423781	1.02108916737011\\
1.58068082442891	1.00656623617291\\
1.62409922462001	1.00179118413672\\
1.66751762481112	1.01959409919452\\
1.71093602500222	1.04345944761309\\
1.75435442519332	1.04409921996373\\
1.79777282538443	1.07989988084049\\
1.84119122557553	1.07933054029004\\
1.88460962576663	1.07904995353667\\
1.92802802595774	1.11292507935232\\
1.97144642614884	1.11392216287114\\
2.01486482633994	1.10504660715487\\
2.05828322653104	1.14084416836161\\
2.10170162672215	1.14068639286384\\
2.14512002691325	1.19211698497447\\
2.18853842710435	1.20090061788986\\
2.23195682729546	1.206864871171\\
2.27537522748656	1.24314127314544\\
2.31879362767766	1.24930433726582\\
2.36221202786877	1.27774490759374\\
2.40563042805987	1.3208190327007\\
2.44904882825097	1.28276473937581\\
2.49246722844208	1.30980417961142\\
2.53588562863318	1.3159139680252\\
2.57930402882428	1.34487757829688\\
2.62272242901538	1.31575634449779\\
2.66614082920649	1.34235504997271\\
2.70955922939759	1.40185500548597\\
2.75297762958869	1.38670289285701\\
2.7963960297798	1.35476862396713\\
2.8398144299709	1.45381339226138\\
2.883232830162	1.50355265518919\\
2.92665123035311	1.48989694124178\\
2.97006963054421	1.55392950261694\\
3.01348803073531	1.62422368253585\\
3.05690643092642	1.66761684763421\\
3.10032483111752	1.5640359082853\\
3.14374323130862	1.71900541123243\\
3.18716163149972	1.82056041475194\\
3.23058003169083	1.87728868020905\\
3.27399843188193	1.89156519728821\\
3.31741683207303	1.88053083166983\\
3.36083523226414	1.70924533265117\\
3.40425363245524	2.04453174240549\\
3.44767203264634	1.90984603192278\\
3.49109043283745	2.05517936669963\\
3.53450883302855	2.08592215984493\\
3.57792723321965	1.97087828318097\\
3.62134563341076	2.00470464283358\\
3.66476403360186	2.10779274546864\\
3.70818243379296	1.94540836482294\\
3.75160083398406	1.83758801479053\\
3.79501923417517	2.04754634486467\\
3.83843763436627	2.08300369451607\\
3.88185603455737	2.4806905383492\\
3.92527443474848	2.5170689512722\\
3.96869283493958	3.3504676710664\\
4.01211123513068	2.82039711372905\\
4.05552963532179	2.28698248011355\\
4.09894803551289	2.66845561495929\\
4.14236643570399	3.47807273804699\\
4.1857848358951	3.51957038768943\\
4.2292032360862	4.31522417123272\\
4.2726216362773	3.54174613586398\\
4.3160400364684	4.20761384205655\\
4.35945843665951	5.35074026902701\\
4.40287683685061	9.04614093988916\\
4.44629523704171	7.69700235063016\\
4.48971363723282	4.28957430082152\\
4.53313203742392	2.69765966695077\\
4.57655043761502	4.60273822914904\\
4.61996883780613	11.6457796597644\\
};
\addlegendentry{$\theta\text{'/}\sigma{}_\theta$}


\addplot [color=black, dashed, line width = 0.5pt]
  table[row sep=crcr]{%
-6	1\\
6	1\\
};
\addlegendentry{\footnotesize Gaussian};

% \addplot[area legend, draw=black, fill=black, fill opacity=0.01]
% table[row sep=crcr] {%
% x	y\\
% -6	0.909090909090\\
% 6	0.909090909090\\
% 6	1.1\\
% -6	1.1\\
% }--cycle;
 \addplot[fill=black, fill opacity = 0.1, draw = none,area legend] coordinates {(-6,0.9090909090) (6,0.9090909090) (6,1.1) (-6,1.1)};
\addlegendentry{\footnotesize $\pm10\%$};

\end{axis}
\begin{axis}[%
width=\Width,
height=\Height,
at={(0in,\VSKIP)},
scale only axis,
xmin=-5.5,
xmax=5.5,
xlabel style={font=\color{white!15!black}},%xlabel={$\text{u'/}\sigma{}_\text{u}\text{    ,  }\theta\text{'/}\sigma{}_\theta$},
ymode=log,
ymin=0.25,
ymax=64, % ymin=0.909090909,% ymax=1.1,
ytick={0.0625, 0.125, 0.25, 0.5, 1, 2, 4, 8, 16, 32, 64}, 
yticklabels={$1/16$, $1/8$, $1/4$, $1/2$ ,$1$, $2$ ,$4$,$8$ , $16$, $32$ , $64$},
xtick={-5,-4,-3,-2,-1,0,1,2,3,4,5}, 
xticklabels={-5,-4,-3,-2,-1,0,1,2,3,4,5},
ticklabel style = {font=\footnotesize} ,
yminorticks=true,
ylabel style={font=\color{white!15!black}, text width=2.5cm},
ylabel= {$\mathrm{PDF}_{exp}/\mathrm{PDF}_{norm}$},% ylabel= {$\mathrm{pdf(u'/\sigma_{u})}_{exp}/\mathrm{pdf}_{norm}$ \\ $\mathrm{pdf(\theta'/\sigma_{\theta})}_{exp}/\mathrm{pdf}_{norm}$},
axis background/.style={fill=white},
ylabel shift = -4pt,
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(1.,0.03)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black,draw=none}
]


\node[fill = white, rotate =0, anchor = center] (z1) at (axis cs:0,32) {$z = 0.125$ m};


\addplot [color=mycolor6, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor6}]
  table[row sep=crcr]{%
-4.860551698549	36.8442268992987\\
-4.80821798771478	8.47848087279959\\
-4.75588427688057	4.89965917136963\\
-4.70355056604636	9.07979246038391\\
-4.65121685521215	10.2754616053657\\
-4.59888314437793	10.5117984093739\\
-4.54654943354372	14.3515073562349\\
-4.49421572270951	9.80287046409075\\
-4.4418820118753	8.65610809257275\\
-4.38954830104108	12.7331577230991\\
-4.33721459020687	12.4744074299288\\
-4.28488087937266	10.0617432971821\\
-4.23254716853845	8.70928160836162\\
-4.18021345770423	9.96292733565959\\
-4.12787974687002	10.263348127939\\
-4.07554603603581	9.8018201479313\\
-4.02321232520159	8.78810883782565\\
-3.97087861436738	7.66091823589692\\
-3.91854490353317	6.80283319123618\\
-3.86621119269896	6.36147075479685\\
-3.81387748186474	6.64562398872174\\
-3.76154377103053	7.59048428824442\\
-3.70921006019632	6.25681607121583\\
-3.65687634936211	5.14238641630829\\
-3.60454263852789	5.43904776095896\\
-3.55220892769368	5.10490226132367\\
-3.49987521685947	4.91864681543105\\
-3.44754150602525	4.81776315419258\\
-3.39520779519104	4.90993719020134\\
-3.34287408435683	4.86031953720358\\
-3.29054037352262	4.46471251292512\\
-3.2382066626884	4.25242884677718\\
-3.18587295185419	4.0139113325752\\
-3.13353924101998	3.70698089332672\\
-3.08120553018577	3.70159097903642\\
-3.02887181935155	3.64824400660712\\
-2.97653810851734	3.4311364453864\\
-2.92420439768313	3.29866151246929\\
-2.87187068684891	3.21955883229334\\
-2.8195369760147	3.11008435919531\\
-2.76720326518049	2.98830916644471\\
-2.71486955434628	2.91259472347876\\
-2.66253584351206	2.94084563671981\\
-2.61020213267785	2.79895140111774\\
-2.55786842184364	2.60319148358082\\
-2.50553471100943	2.56879861892368\\
-2.45320100017521	2.43051334081354\\
-2.400867289341	2.411048569994\\
-2.34853357850679	2.32260855943051\\
-2.29619986767257	2.22904413896699\\
-2.24386615683836	2.12755262605173\\
-2.19153244600415	2.038398709321\\
-2.13919873516994	1.93055012190403\\
-2.08686502433572	1.91004858084444\\
-2.03453131350151	1.88343598364016\\
-1.9821976026673	1.8144335855068\\
-1.92986389183309	1.75773101497444\\
-1.87753018099887	1.67392095276024\\
-1.82519647016466	1.63796037729432\\
-1.77286275933045	1.59426199440507\\
-1.72052904849624	1.54092776827423\\
-1.66819533766202	1.47859012166983\\
-1.61586162682781	1.43731711800385\\
-1.5635279159936	1.40166946277916\\
-1.51119420515938	1.38545109351289\\
-1.45886049432517	1.34663787055203\\
-1.40652678349096	1.31464386231598\\
-1.35419307265675	1.28742827546668\\
-1.30185936182253	1.23993865365118\\
-1.24952565098832	1.19523540141589\\
-1.19719194015411	1.18220181421306\\
-1.1448582293199	1.15652449940278\\
-1.09252451848568	1.13095761166966\\
-1.04019080765147	1.10554134554121\\
-0.987857096817258	1.07675350639848\\
-0.935523385983045	1.04151984387888\\
-0.883189675148832	1.02945499520859\\
-0.830855964314619	0.999736646610459\\
-0.778522253480407	0.980057002664146\\
-0.726188542646194	0.95775126123526\\
-0.673854831811981	0.937957728753368\\
-0.621521120977768	0.92430435094948\\
-0.569187410143556	0.918141004371009\\
-0.516853699309343	0.920085073861593\\
-0.46451998847513	0.901326799223285\\
-0.412186277640918	0.888505198855229\\
-0.359852566806705	0.872612993492079\\
-0.307518855972492	0.859860836026456\\
-0.25518514513828	0.846892225092139\\
-0.202851434304067	0.842237108741234\\
-0.150517723469855	0.831585433398412\\
-0.0981840126356416	0.816497338261942\\
-0.0458503018014291	0.816488394117565\\
0.00648340903278372	0.811803115320559\\
0.0588171198669963	0.809461535418938\\
0.111150830701209	0.809391538347072\\
0.163484541535422	0.808131433595815\\
0.215818252369635	0.804375755010618\\
0.268151963203847	0.798919408065948\\
0.32048567403806	0.79905454014666\\
0.372819384872273	0.808936753885087\\
0.425153095706485	0.817530063558885\\
0.477486806540698	0.817063640071719\\
0.529820517374911	0.822358678201337\\
0.582154228209123	0.820547836167066\\
0.634487939043336	0.83012212447307\\
0.686821649877549	0.839875297341288\\
0.739155360711761	0.85001079028683\\
0.791489071545974	0.854092337702107\\
0.843822782380187	0.865254115172337\\
0.8961564932144	0.880548534367243\\
0.948490204048612	0.895332972340615\\
1.00082391488283	0.904525384715808\\
1.05315762571704	0.926617190306589\\
1.10549133655125	0.94881580293123\\
1.15782504738546	0.966491036852275\\
1.21015875821968	0.996615675200806\\
1.26249246905389	1.00878997471362\\
1.3148261798881	1.02658665863475\\
1.36715989072231	1.04280257347086\\
1.41949360155653	1.05127967582773\\
1.47182731239074	1.08666238301969\\
1.52416102322495	1.1124578548504\\
1.57649473405916	1.15825549014708\\
1.62882844489338	1.17454727021053\\
1.68116215572759	1.21626250055121\\
1.7334958665618	1.21842583173946\\
1.78582957739602	1.24082908623761\\
1.83816328823023	1.26620456756095\\
1.89049699906444	1.29844753217774\\
1.94283070989865	1.33999026095487\\
1.99516442073287	1.41425362607049\\
2.04749813156708	1.42372178633383\\
2.09983184240129	1.44509570382268\\
2.1521655532355	1.44573854318699\\
2.20449926406972	1.51072611926425\\
2.25683297490393	1.62117150624588\\
2.30916668573814	1.68297441896302\\
2.36150039657235	1.68671019099091\\
2.41383410740657	1.7388275715152\\
2.46616781824078	1.80160027956707\\
2.51850152907499	1.83788804260607\\
2.57083523990921	1.96574789423207\\
2.62316895074342	2.0598218020794\\
2.67550266157763	2.2543549404168\\
2.72783637241184	2.26999939252157\\
2.78017008324606	2.37726871201893\\
2.83250379408027	2.48647631036464\\
2.88483750491448	2.60265073509375\\
2.93717121574869	2.83375928894119\\
2.98950492658291	2.81864608933748\\
3.04183863741712	2.91940988653642\\
3.09417234825133	3.21586227085096\\
3.14650605908555	3.25987148463295\\
3.19883976991976	3.70330335896661\\
3.25117348075397	4.12452229691736\\
3.30350719158818	4.3828824854143\\
3.3558409024224	4.4530125653765\\
3.40817461325661	4.53896665410723\\
3.46050832409082	5.0898182449466\\
3.51284203492503	5.71434673807983\\
3.56517574575925	5.59218683788371\\
3.61750945659346	6.12759517255709\\
3.66984316742767	6.28225787066654\\
3.72217687826189	7.13467836825492\\
3.7745105890961	6.55807698409516\\
3.82684429993031	6.94678489515757\\
3.87917801076452	8.59040500680275\\
3.93151172159874	9.44463043303978\\
3.98384543243295	10.7420826693741\\
4.03617914326716	12.7039661340718\\
4.08851285410137	12.2416602139292\\
4.14084656493559	14.2045094399911\\
4.1931802757698	13.728236236602\\
4.24551398660401	16.7248982946336\\
4.29784769743822	24.6336432312823\\
4.35018140827244	16.516123442427\\
4.40251511910665	21.4702039410052\\
4.45484882994086	26.2711311830872\\
4.50718254077507	26.5487038677022\\
4.55951625160929	21.1365095689218\\
4.6118499624435	26.3119964012698\\
4.66418367327771	30.0460817398154\\
4.71651738411193	30.461062058067\\
4.76885109494614	40.2932304180422\\
4.82118480578035	28.5013271466778\\
4.87351851661456	36.6408842558061\\
4.92585222744878	47.566040607869\\
4.97818593828299	33.7182217380146\\
5.0305196491172	67.5598856660683\\
5.08285335995141	52.3987910095208\\
5.13518707078563	143.623133167871\\
5.18752078161984	485.62183083435\\
5.23985449245405	206.971306444473\\
5.29218820328827	39.2131093034498\\
5.34452191412248	64.263084317461\\
5.39685562495669	51.5167374226461\\
5.4491893357909	142.339205974089\\
5.50152304662512	258.7478730347\\
5.55385675745933	1074.0379156008\\
};
\addlegendentry{$\text{u'/}\sigma{}_\text{u}$}

\addplot [color=mycolor5, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor5}]
  table[row sep=crcr]{%
-4.36755971515259	4.38292135680342\\
-4.3212490572506	2.05270191347054\\
-4.27493839934862	1.53907820191235\\
-4.22862774144664	1.98448834894408\\
-4.18231708354465	1.08454234950661\\
-4.13600642564267	0.84828332090653\\
-4.08969576774068	1.0411683398288\\
-4.0433851098387	1.14356751099417\\
-3.99707445193671	0.773486149139089\\
-3.95076379403473	1.19811154366336\\
-3.90445313613274	1.07354848090665\\
-3.85814247823076	1.25441881883365\\
-3.81183182032877	1.45892850065407\\
-3.76552116242679	1.96624374620708\\
-3.7192105045248	2.05458732974027\\
-3.67289984662282	2.46143378553334\\
-3.62658918872083	2.52583086752403\\
-3.58027853081885	2.37815479691167\\
-3.53396787291686	2.08925260154448\\
-3.48765721501488	2.14425389423221\\
-3.44134655711289	2.2783786679666\\
-3.39503589921091	2.39573060941747\\
-3.34872524130892	2.56061890759844\\
-3.30241458340694	2.38891165079013\\
-3.25610392550495	2.29002146341544\\
-3.20979326760297	2.31539521429936\\
-3.16348260970098	2.57386698681198\\
-3.117171951799	2.37437898941261\\
-3.07086129389702	2.4365537163399\\
-3.02455063599503	2.37248037089985\\
-2.97823997809305	2.28332284571689\\
-2.93192932019106	2.19567321634205\\
-2.88561866228908	2.18214413755737\\
-2.83930800438709	2.28019078507598\\
-2.79299734648511	2.23423967866633\\
-2.74668668858312	2.08742782665571\\
-2.70037603068114	1.98924962631816\\
-2.65406537277915	2.02873051692911\\
-2.60775471487717	2.0108207609594\\
-2.56144405697518	2.02866950305461\\
-2.5151333990732	1.96312827163359\\
-2.46882274117121	1.84482567093839\\
-2.42251208326923	1.76692253732904\\
-2.37620142536724	1.77677875284633\\
-2.32989076746526	1.75009436204011\\
-2.28358010956327	1.71146308860025\\
-2.23726945166129	1.61483892316087\\
-2.1909587937593	1.5639131864091\\
-2.14464813585732	1.59193151514132\\
-2.09833747795533	1.52907713112264\\
-2.05202682005335	1.47806999259993\\
-2.00571616215136	1.43485470755267\\
-1.95940550424938	1.41003073671819\\
-1.91309484634739	1.34741726165301\\
-1.86678418844541	1.36749688903108\\
-1.82047353054342	1.34224494484053\\
-1.77416287264144	1.25831480645926\\
-1.72785221473946	1.26635788418913\\
-1.68154155683747	1.26345797070161\\
-1.63523089893549	1.24104819295816\\
-1.5889202410335	1.1958216863083\\
-1.54260958313152	1.17512755186209\\
-1.49629892522953	1.16221353329279\\
-1.44998826732755	1.15343356860639\\
-1.40367760942556	1.13117300132339\\
-1.35736695152358	1.09960772046864\\
-1.31105629362159	1.082652953741\\
-1.26474563571961	1.0745739523156\\
-1.21843497781762	1.07398821840241\\
-1.17212431991564	1.04053109640938\\
-1.12581366201365	1.01981898662068\\
-1.07950300411167	1.01295470709958\\
-1.03319234620968	0.998154719121442\\
-0.986881688307699	0.991854653421188\\
-0.940571030405714	0.980285410418573\\
-0.894260372503729	0.973335041502275\\
-0.847949714601744	0.965681639599089\\
-0.801639056699759	0.955511586379676\\
-0.755328398797774	0.958218760216542\\
-0.70901774089579	0.965053469067445\\
-0.662707082993805	0.936263048184057\\
-0.61639642509182	0.925637919840285\\
-0.570085767189835	0.930124938116723\\
-0.523775109287851	0.924398756014882\\
-0.477464451385866	0.929691103736543\\
-0.431153793483881	0.930477900746458\\
-0.384843135581896	0.930384871143981\\
-0.338532477679911	0.921556687052239\\
-0.292221819777926	0.922219699406555\\
-0.245911161875942	0.905352484828965\\
-0.199600503973957	0.911682421628324\\
-0.153289846071972	0.926955836475942\\
-0.106979188169987	0.915284012041628\\
-0.0606685302680023	0.909307834093679\\
-0.0143578723660176	0.916088905297619\\
0.031952785535967	0.917138370290224\\
0.0782634434379516	0.91699826369701\\
0.124574101339937	0.920862076382901\\
0.170884759241921	0.918798790706024\\
0.217195417143906	0.927114465961636\\
0.263506075045891	0.928275825291508\\
0.309816732947876	0.92499320992186\\
0.356127390849861	0.934189488639237\\
0.402438048751846	0.933653760072264\\
0.44874870665383	0.938769911435051\\
0.495059364555815	0.939022101200606\\
0.5413700224578	0.953695240396581\\
0.587680680359785	0.956744020271937\\
0.63399133826177	0.964164883795553\\
0.680301996163754	0.963026573213555\\
0.726612654065739	0.965364791915446\\
0.772923311967724	0.964024467283251\\
0.819233969869709	0.981844043042175\\
0.865544627771694	0.990383180981857\\
0.911855285673678	1.00051138400479\\
0.958165943575664	1.00116666110939\\
1.00447660147765	1.00933417658963\\
1.05078725937963	1.02327713063164\\
1.09709791728162	1.03405895671487\\
1.1434085751836	1.02588494940835\\
1.18971923308559	1.03903367414905\\
1.23602989098757	1.045321680344\\
1.28234054888956	1.04048989613871\\
1.32865120679154	1.07829305487271\\
1.37496186469353	1.0806197354692\\
1.42127252259551	1.07468925575836\\
1.4675831804975	1.07525120021827\\
1.51389383839948	1.07127376000105\\
1.56020449630147	1.07701731877009\\
1.60651515420345	1.08372755384067\\
1.65282581210544	1.10702969782284\\
1.69913647000742	1.1265462618505\\
1.7454471279094	1.11964671761876\\
1.79175778581139	1.12910478739512\\
1.83806844371337	1.12625101323637\\
1.88437910161536	1.1279443891836\\
1.93068975951734	1.13972729507199\\
1.97700041741933	1.18720308561246\\
2.02331107532131	1.19549428678842\\
2.0696217332233	1.19211630244144\\
2.11593239112528	1.18820351597201\\
2.16224304902727	1.18946803467231\\
2.20855370692925	1.19931279079381\\
2.25486436483124	1.20725161945378\\
2.30117502273322	1.20144351928871\\
2.34748568063521	1.20972361760241\\
2.39379633853719	1.24639550411424\\
2.44010699643918	1.29770071237523\\
2.48641765434116	1.30163150409066\\
2.53272831224315	1.303255347462\\
2.57903897014513	1.36086866224068\\
2.62534962804712	1.34941715116773\\
2.6716602859491	1.34552050890205\\
2.71797094385109	1.37435385088923\\
2.76428160175307	1.28467004070748\\
2.81059225965506	1.30321598695837\\
2.85690291755704	1.28636887733454\\
2.90321357545902	1.37601600420094\\
2.94952423336101	1.45689487909069\\
2.99583489126299	1.57902806570856\\
3.04214554916498	1.55441670393166\\
3.08845620706696	1.5197123687683\\
3.13476686496895	1.52900976686973\\
3.18107752287093	1.53363337049341\\
3.22738818077292	1.62932942581715\\
3.2736988386749	1.7294295463387\\
3.32000949657689	1.68388529367211\\
3.36632015447887	1.98364355799848\\
3.41263081238086	1.86498083425379\\
3.45894147028284	1.71042598231242\\
3.50525212818483	2.07630867648239\\
3.55156278608681	2.04826170182755\\
3.5978734439888	1.87600380756715\\
3.64418410189078	1.87850709362784\\
3.69049475979277	1.97336876782486\\
3.73680541769475	2.2147900111789\\
3.78311607559674	1.85577650976018\\
3.82942673349872	2.47377536786875\\
3.87573739140071	2.8877571869949\\
3.92204804930269	2.81120160432625\\
3.96835870720468	2.77000688495539\\
4.01466936510666	2.6118519912476\\
4.06098002300864	2.40177482529855\\
4.10729068091063	2.29039443163371\\
4.15360133881262	2.48134271902891\\
4.1999119967146	2.65881534761359\\
4.24622265461658	3.12101471996246\\
4.29253331251857	2.71680097467167\\
4.33884397042055	3.48114770553597\\
4.38515462832254	3.15675026268022\\
4.43146528622452	2.00725697820564\\
4.47777594412651	3.0849289498584\\
4.52408660202849	2.41592129635564\\
4.57039725993048	1.83748188511543\\
4.61670791783246	1.79450305756125\\
4.66301857573445	5.71169015435604\\
4.70932923363643	2.45643572006272\\
4.75563989153842	5.56148885383769\\
4.8019505494404	13.152256402012\\
4.84826120734239	32.579667216727\\
};
\addlegendentry{$\theta\text{'/}\sigma{}_\theta$}


\addplot [color=black, dashed, line width = 0.5pt]
  table[row sep=crcr]{%
-6	1\\
6	1\\
};
\addlegendentry{\footnotesize Gaussian};

% \addplot[area legend, draw=black, fill=black, fill opacity=0.01]
% table[row sep=crcr] {%
% x	y\\
% -6	0.909090909090\\
% 6	0.909090909090\\
% 6	1.1\\
% -6	1.1\\
% }--cycle;
 \addplot[fill=black, fill opacity = 0.1, draw = none,area legend] coordinates {(-6,0.9090909090) (6,0.9090909090) (6,1.1) (-6,1.1)};
\addlegendentry{\footnotesize $\pm10\%$};

\end{axis}
\begin{axis}[%
width=\Width,
height=\Height,
at={(0in,0in)},
scale only axis,
xmin=-5.5,
xmax=5.5,
xlabel style={font=\color{white!15!black}},
xlabel={$u'\sigma{}_\text{u}\text{    ,  }\theta'\sigma{}_\theta$},
ymode=log,
ymin=0.25,
ymax=64, % ymin=0.909090909,% ymax=1.1,
ytick={0.0625, 0.125, 0.25, 0.5, 1, 2, 4, 8, 16, 32, 64}, 
yticklabels={$1/16$, $1/8$, $1/4$, $1/2$ ,$1$, $2$ ,$4$,$8$ , $16$, $32$ , $64$},
xtick={-5,-4,-3,-2,-1,0,1,2,3,4,5}, 
xticklabels={-5,-4,-3,-2,-1,0,1,2,3,4,5},
ticklabel style = {font=\footnotesize} ,
yminorticks=true,
ylabel style={font=\color{white!15!black}, text width=2.5cm},
ylabel= {$\mathrm{PDF}_{exp}/\mathrm{PDF}_{norm}$},% ylabel= {$\mathrm{pdf(u'/\sigma_{u})}_{exp}/\mathrm{pdf}_{norm}$ \\ $\mathrm{pdf(\theta'/\sigma_{\theta})}_{exp}/\mathrm{pdf}_{norm}$},
axis background/.style={fill=white},
ylabel shift = -4pt,
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(1.,0.03)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black,draw=none}
]
\node[fill = white, rotate =0, anchor = center] (z1) at (axis cs:0,32) {$z = 0.0625$ m};

\addplot [color=mycolor8, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor8}]
  table[row sep=crcr]{%
-4.12658275808832	1.86653009274671\\
-4.07424631366351	1.17367265357447\\
-4.02190986923869	0.736938882927558\\
-3.96957342481388	0.737742357635525\\
-3.91723698038906	0.828222687455887\\
-3.86490053596424	0.717963029917197\\
-3.81256409153943	0.75580038454552\\
-3.76022764711461	1.10847286769618\\
-3.7078912026898	0.922883732332492\\
-3.65555475826498	0.951134176439066\\
-3.60321831384017	0.948025429956758\\
-3.55088186941535	0.950926127212651\\
-3.49854542499053	1.21827161028606\\
-3.44620898056572	1.06395222340271\\
-3.3938725361409	1.01608324534551\\
-3.34153609171609	1.11975208385073\\
-3.28919964729127	1.1169032356437\\
-3.23686320286645	1.05895405219506\\
-3.18452675844164	1.0954613369049\\
-3.13219031401682	1.10284096979236\\
-3.07985386959201	1.11614095960627\\
-3.02751742516719	1.23738419070727\\
-2.97518098074237	1.09711475946206\\
-2.92284453631756	1.04743425360903\\
-2.87050809189274	1.13112906291152\\
-2.81817164746793	1.16667065511952\\
-2.76583520304311	1.19311267145174\\
-2.71349875861829	1.24346574086472\\
-2.66116231419348	1.25996315327795\\
-2.60882586976866	1.1694646009631\\
-2.55648942534385	1.18660044858954\\
-2.50415298091903	1.19438232862994\\
-2.45181653649422	1.25445493826201\\
-2.3994800920694	1.25200286659255\\
-2.34714364764458	1.22782372983572\\
-2.29480720321977	1.22798024708691\\
-2.24247075879495	1.27497454053518\\
-2.19013431437014	1.29802012998389\\
-2.13779786994532	1.28759777980533\\
-2.0854614255205	1.27687801566664\\
-2.03312498109569	1.2683961415954\\
-1.98078853667087	1.27535760861798\\
-1.92845209224606	1.25815557288713\\
-1.87611564782124	1.25101658842851\\
-1.82377920339642	1.27906358157061\\
-1.77144275897161	1.27146814062373\\
-1.71910631454679	1.23831607610797\\
-1.66676987012198	1.23161383553524\\
-1.61443342569716	1.2448294268853\\
-1.56209698127234	1.23007222615715\\
-1.50976053684753	1.21502519188496\\
-1.45742409242271	1.17893532547954\\
-1.4050876479979	1.17338759797704\\
-1.35275120357308	1.17823437659107\\
-1.30041475914826	1.1647675553123\\
-1.24807831472345	1.1634539996735\\
-1.19574187029863	1.15496297180976\\
-1.14340542587382	1.1264955830972\\
-1.091068981449	1.11867907547357\\
-1.03873253702419	1.10712979597157\\
-0.98639609259937	1.09689335886828\\
-0.934059648174554	1.08666359070589\\
-0.881723203749738	1.06838512121701\\
-0.829386759324922	1.05875261857876\\
-0.777050314900106	1.05245276840722\\
-0.72471387047529	1.0476201625097\\
-0.672377426050474	1.02821395611625\\
-0.620040981625658	1.01045228957717\\
-0.567704537200842	1.01034049957297\\
-0.515368092776026	0.995184640266654\\
-0.46303164835121	0.98606988035647\\
-0.410695203926394	0.981245593523472\\
-0.358358759501578	0.97518477903536\\
-0.306022315076762	0.981074110534321\\
-0.253685870651947	0.976365261361665\\
-0.201349426227131	0.963624745753158\\
-0.149012981802315	0.967005530586832\\
-0.096676537377499	0.966064576319394\\
-0.0443400929526828	0.958941547167395\\
0.00799635147213285	0.947667397741958\\
0.060332795896949	0.943895857483646\\
0.112669240321765	0.941586831766788\\
0.165005684746581	0.936068798454443\\
0.217342129171397	0.932108706981639\\
0.269678573596213	0.925142938341679\\
0.322015018021028	0.926430482702527\\
0.374351462445844	0.930001872458317\\
0.42668790687066	0.92182345662704\\
0.479024351295476	0.926567750394652\\
0.531360795720292	0.936442986409338\\
0.583697240145108	0.936977470425163\\
0.636033684569924	0.929045012642367\\
0.68837012899474	0.917593444757643\\
0.740706573419556	0.916824393630192\\
0.793043017844372	0.924748554605061\\
0.845379462269187	0.932012285686043\\
0.897715906694003	0.943096269625904\\
0.950052351118819	0.940828141479564\\
1.00238879554364	0.940113517174892\\
1.05472523996845	0.945745494128762\\
1.10706168439327	0.94350241759922\\
1.15939812881808	0.955768260870435\\
1.2117345732429	0.957865058577545\\
1.26407101766771	0.946549770914806\\
1.31640746209253	0.962856835902157\\
1.36874390651735	0.963127688495944\\
1.42108035094216	0.963089914113794\\
1.47341679536698	0.973265240658849\\
1.52575323979179	0.982709587164739\\
1.57808968421661	0.97701202357858\\
1.63042612864143	0.98816059641381\\
1.68276257306624	0.993728737232458\\
1.73509901749106	0.990775162857251\\
1.78743546191587	0.991882101521809\\
1.83977190634069	1.02868051655306\\
1.89210835076551	1.05126295976836\\
1.94444479519032	1.05117085639849\\
1.99678123961514	1.03695617696604\\
2.04911768403995	1.08207533607931\\
2.10145412846477	1.11605453324945\\
2.15379057288959	1.12065432707301\\
2.2061270173144	1.13254941689556\\
2.25846346173922	1.17037173266064\\
2.31079990616403	1.15906943664859\\
2.36313635058885	1.18440314378323\\
2.41547279501366	1.1980058074759\\
2.46780923943848	1.2477394148523\\
2.5201456838633	1.29022666039079\\
2.57248212828811	1.34996842127184\\
2.62481857271293	1.40027416521069\\
2.67715501713774	1.46340758695456\\
2.72949146156256	1.50602934035001\\
2.78182790598738	1.49007375448317\\
2.83416435041219	1.57005223919686\\
2.88650079483701	1.48217325891633\\
2.93883723926182	1.63287927853914\\
2.99117368368664	1.79023041524365\\
3.04351012811146	1.90616652104669\\
3.09584657253627	1.91005246015996\\
3.14818301696109	1.98778630211482\\
3.2005194613859	2.26859626158591\\
3.25285590581072	2.33155901765428\\
3.30519235023554	2.41343025810636\\
3.35752879466035	2.46944240703057\\
3.40986523908517	2.6349637510805\\
3.46220168350998	2.88656447001968\\
3.5145381279348	3.51444021709764\\
3.56687457235962	3.58442274949724\\
3.61921101678443	3.82554519566429\\
3.67154746120925	4.52448807492525\\
3.72388390563406	4.78505670403142\\
3.77622035005888	5.4444005845398\\
3.8285567944837	5.6256267858755\\
3.88089323890851	5.99657377321746\\
3.93322968333333	7.54981907852313\\
3.98556612775814	9.01510143894633\\
4.03790257218296	8.64189250301472\\
4.09023901660777	8.59579242261761\\
4.14257546103259	10.5132320155968\\
4.19491190545741	9.73260041114376\\
4.24724834988222	11.4372490426908\\
4.29958479430704	11.4561345559531\\
4.35192123873185	15.4968094766621\\
4.40425768315667	21.0190571246395\\
4.45659412758149	21.2362247196199\\
4.5089305720063	18.7143595653908\\
4.56126701643112	30.3571241131285\\
4.61360346085593	28.4498439886443\\
4.66593990528075	41.738172486483\\
4.71827634970556	45.8416843248386\\
4.77061279413038	47.0140300751288\\
4.8229492385552	45.0343741053297\\
4.87528568298001	62.1505529588404\\
4.92762212740483	81.7297515137223\\
4.97995857182965	72.8453105084206\\
5.03229501625446	96.4967399883942\\
5.08463146067928	152.141384296929\\
5.13696790510409	116.467125197379\\
5.18930434952891	156.977319972954\\
5.24164079395372	88.9737495678392\\
5.29397723837854	104.337722117799\\
5.34631368280336	193.041405821393\\
5.39865012722817	135.286163618579\\
5.45098657165299	69.53449767548\\
5.5033230160778	239.185878485269\\
5.55565946050262	273.695127453809\\
5.60799590492744	274.791500085989\\
5.66033234935225	1167.83271040484\\
5.71266879377707	1397.15890283453\\
5.76500523820188	294.056277035293\\
5.8173416826267	0\\
5.86967812705152	853.213119489288\\
5.92201457147633	3421.71871535863\\
5.97435101590115	1777.81102680032\\
6.02668746032596	3707.99966779848\\
6.07902390475078	2569.843499906\\
6.1313603491756	6598.07908124202\\
6.18369679360041	1645.24559259497\\
6.23603323802523	17271.887554895\\
6.28836968245004	83091.7069684693\\
};
\addlegendentry{$\text{u'/}\sigma{}_\text{u}$}




\addplot [color=mycolor7, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor7}]
  table[row sep=crcr]{%
-3.87822575924531	0.696019913646553\\
-3.83214113154068	0.26814916144231\\
-3.78605650383605	0.273657976016474\\
-3.73997187613142	0.344896274060428\\
-3.69388724842679	0.35928536344527\\
-3.64780262072216	0.20734211526664\\
-3.60171799301753	0.322829108603373\\
-3.55563336531291	0.432697288442152\\
-3.50954873760828	0.51097805546516\\
-3.46346410990365	0.492268369480417\\
-3.41737948219902	0.552480328250371\\
-3.37129485449439	0.617794975033102\\
-3.32521022678976	0.580159377674328\\
-3.27912559908513	0.538735374240201\\
-3.2330409713805	0.393299367275304\\
-3.18695634367587	0.533507019785443\\
-3.14087171597124	0.634933226369558\\
-3.09478708826661	0.67903367654058\\
-3.04870246056198	0.685146236828986\\
-3.00261783285736	0.741057077421685\\
-2.95653320515273	0.827237197796896\\
-2.9104485774481	0.824728504539346\\
-2.86436394974347	0.837960568144341\\
-2.81827932203884	0.859922907569803\\
-2.77219469433421	0.895422000098484\\
-2.72611006662958	0.958832775908504\\
-2.68002543892495	0.985946560671348\\
-2.63394081122032	0.934401857613637\\
-2.58785618351569	1.00567430417257\\
-2.54177155581106	1.05846026472658\\
-2.49568692810644	1.01336672122206\\
-2.44960230040181	1.05212821377208\\
-2.40351767269718	1.08619303108356\\
-2.35743304499255	1.12127645848185\\
-2.31134841728792	1.06257230434169\\
-2.26526378958329	1.05729448512101\\
-2.21917916187866	1.12310725828602\\
-2.17309453417403	1.15582527888125\\
-2.1270099064694	1.16545486145154\\
-2.08092527876477	1.15851702098647\\
-2.03484065106015	1.18728503320253\\
-1.98875602335552	1.17826669463442\\
-1.94267139565089	1.17049260692023\\
-1.89658676794626	1.18797661971181\\
-1.85050214024163	1.18089395190144\\
-1.804417512537	1.2034729350307\\
-1.75833288483237	1.20200874785309\\
-1.71224825712774	1.18509792942233\\
-1.66616362942311	1.17430947504401\\
-1.62007900171848	1.15454534136289\\
-1.57399437401385	1.15581669258939\\
-1.52790974630923	1.15759705263982\\
-1.4818251186046	1.15495467268407\\
-1.43574049089997	1.1441097959327\\
-1.38965586319534	1.13573917585099\\
-1.34357123549071	1.124972297107\\
-1.29748660778608	1.1141372159807\\
-1.25140198008145	1.12413397390341\\
-1.20531735237682	1.10382791298482\\
-1.15923272467219	1.08025338792723\\
-1.11314809696756	1.07767936742565\\
-1.06706346926293	1.07981549570928\\
-1.02097884155831	1.07598203406794\\
-0.974894213853676	1.07185183011182\\
-0.928809586149047	1.06179921904876\\
-0.882724958444418	1.04654243172612\\
-0.836640330739789	1.05465990812585\\
-0.79055570303516	1.05441632222847\\
-0.744471075330531	1.05481487621712\\
-0.698386447625902	1.03435945734771\\
-0.652301819921273	1.02675088388348\\
-0.606217192216644	1.0190191951827\\
-0.560132564512015	1.01894326457699\\
-0.514047936807386	1.01934351925305\\
-0.467963309102756	1.00993275684737\\
-0.421878681398128	0.998113727137011\\
-0.375794053693498	0.982669872858878\\
-0.329709425988869	0.975356219230589\\
-0.28362479828424	0.972088381751423\\
-0.237540170579611	0.967238855741769\\
-0.191455542874982	0.96619274082058\\
-0.145370915170353	0.962139678227135\\
-0.0992862874657242	0.956068897201557\\
-0.0532016597610948	0.950988977556264\\
-0.0071170320564658	0.935265745784063\\
0.0389675956481632	0.930606448963925\\
0.0850522233527922	0.930496583824567\\
0.131136851057422	0.93065977814688\\
0.17722147876205	0.939312456781055\\
0.22330610646668	0.932930414046404\\
0.269390734171308	0.933497078833484\\
0.315475361875938	0.925398211497895\\
0.361559989580567	0.910560321587887\\
0.407644617285196	0.91213135759527\\
0.453729244989825	0.916183892264755\\
0.499813872694454	0.908071646373362\\
0.545898500399083	0.900508450785953\\
0.591983128103712	0.910328487476417\\
0.638067755808341	0.89371920669227\\
0.68415238351297	0.901266804985372\\
0.730237011217599	0.919270929793132\\
0.776321638922228	0.907089056058057\\
0.822406266626858	0.907612092188734\\
0.868490894331487	0.913494547490822\\
0.914575522036116	0.919784681018057\\
0.960660149740745	0.912866225803555\\
1.00674477744537	0.914095522997676\\
1.05282940515	0.919999781585173\\
1.09891403285463	0.917408596362517\\
1.14499866055926	0.925344216381554\\
1.19108328826389	0.944711080799182\\
1.23716791596852	0.946123064835705\\
1.28325254367315	0.953896521254892\\
1.32933717137778	0.956972482761784\\
1.37542179908241	0.973542197101693\\
1.42150642678704	0.974807418846631\\
1.46759105449167	0.98851414727105\\
1.51367568219629	1.00710572264877\\
1.55976030990092	1.01396935536979\\
1.60584493760555	1.01877672296313\\
1.65192956531018	1.0209952231219\\
1.69801419301481	1.03856402560746\\
1.74409882071944	1.06669943086646\\
1.79018344842407	1.09200279722963\\
1.8362680761287	1.11763714592198\\
1.88235270383333	1.12965991422109\\
1.92843733153796	1.14667328834216\\
1.97452195924258	1.17664776600944\\
2.02060658694721	1.20640122014328\\
2.06669121465184	1.2015103418157\\
2.11277584235647	1.23116742604364\\
2.1588604700611	1.27742277029678\\
2.20494509776573	1.26225394518923\\
2.25102972547036	1.29763182157264\\
2.29711435317499	1.3742046776993\\
2.34319898087962	1.47060177753164\\
2.38928360858425	1.50683477806436\\
2.43536823628887	1.51998459413917\\
2.4814528639935	1.50509186989373\\
2.52753749169813	1.55035054528094\\
2.57362211940276	1.61505701777669\\
2.61970674710739	1.61273991945866\\
2.66579137481202	1.69711611868724\\
2.71187600251665	1.75969552473415\\
2.75796063022128	1.79891563303844\\
2.80404525792591	1.90743655665455\\
2.85012988563054	1.92169830831824\\
2.89621451333517	2.01445448647949\\
2.9422991410398	2.18204707492333\\
2.98838376874442	2.22130987030273\\
3.03446839644905	2.29552405582202\\
3.08055302415368	2.45021020227234\\
3.12663765185831	2.74513018129252\\
3.17272227956294	2.83624408325293\\
3.21880690726757	2.83349007708311\\
3.2648915349722	2.94975450260418\\
3.31097616267683	3.46940875109552\\
3.35706079038146	3.38413879322846\\
3.40314541808609	3.7370288197837\\
3.44923004579072	3.84988042056492\\
3.49531467349534	3.70012380491524\\
3.54139930119997	4.09757736205377\\
3.5874839289046	4.45425914681825\\
3.63356855660923	4.66902439629355\\
3.67965318431386	4.8793908421996\\
3.72573781201849	5.62771291315921\\
3.77182243972312	6.16427352425432\\
3.81790706742775	6.27112338496815\\
3.86399169513238	6.59413438482178\\
3.91007632283701	6.15262402656134\\
3.95616095054163	6.48539161350118\\
4.00224557824626	8.64890322506782\\
4.04833020595089	9.24547236536868\\
4.09441483365552	8.10127929595257\\
4.14049946136015	7.55559450516723\\
4.18658408906478	7.14339507624031\\
4.23266871676941	6.76642139544883\\
4.27875334447404	8.37237846052189\\
4.32483797217867	11.3553070879562\\
4.3709225998833	12.150946949422\\
4.41700722758792	17.4455263578055\\
4.46309185529255	21.5195406119126\\
4.50917648299718	24.4132303289235\\
4.55526111070181	19.4678854745344\\
4.60134573840644	19.8351032172898\\
4.64743036611107	19.6921063611376\\
4.6935149938157	20.5767402439498\\
4.73959962152033	17.4077885304139\\
4.78568424922496	28.1841038268499\\
4.83176887692959	17.4339592946739\\
4.87785350463422	9.87942036672192\\
4.92393813233885	28.0140521880974\\
4.97002276004347	10.6965556275634\\
5.0161073877481	28.852082751178\\
5.06219201545273	65.2514053537038\\
5.10827664315736	65.4672558354785\\
5.15436127086199	123.269276486748\\
5.20044589856662	29.3610359514365\\
5.24653052627125	75.2839601167235\\
5.29261515397588	362.1765561849\\
};
\addlegendentry{$\theta\text{'/}\sigma{}_\theta$}

\addplot [color=black, dashed, line width = 0.5pt]
  table[row sep=crcr]{%
-6	1\\
6	1\\
};
\addlegendentry{\footnotesize Gaussian};

% \addplot[area legend, draw=black, fill=black, fill opacity=0.01]
% table[row sep=crcr] {%
% x	y\\
% -6	0.909090909090\\
% 6	0.909090909090\\
% 6	1.1\\
% -6	1.1\\
% }--cycle;
 \addplot[fill=black, fill opacity = 0.1, draw = none,area legend] coordinates {(-6,0.9090909090) (6,0.9090909090) (6,1.1) (-6,1.1)};
\addlegendentry{\footnotesize $\pm10\%$};

\end{axis}
\end{tikzpicture}%








% \begin{axis}[%
% width=2in,
% height=2in,
% at={(.0in,0in)},
% scale only axis,
% xmin=-5.5,
% xmax=5.5,
% xlabel style={font=\color{white!15!black}},
% xlabel={$\text{u'/}\sigma{}_\text{u}\text{    ,  }\theta\text{'/}\sigma{}_\theta$},
% ymode=log,
% ymin=0.25,
% ymax=64, % ymin=0.909090909,% ymax=1.1,
% ytick={0.0625, 0.125, 0.25, 0.5, 1, 2, 4, 8, 16, 32, 64}, 
% yticklabels={$1/16$, $1/8$, $1/4$, $1/2$ ,$1$, $2$ ,$4$,$8$ , $16$, $32$ , $64$},
% xtick={-5,-4,-3,-2,-1,0,1,2,3,4,5}, 
% xticklabels={-5,-4,-3,-2,-1,0,1,2,3,4,5},
% ticklabel style = {font=\footnotesize} ,
% yminorticks=true,
% ylabel style={font=\color{white!15!black}, text width=2.5cm},
% ylabel= {$\mathrm{PDF}_{exp}/\mathrm{PDF}_{norm}$},% ylabel= {$\mathrm{pdf(u'/\sigma_{u})}_{exp}/\mathrm{pdf}_{norm}$ \\ $\mathrm{pdf(\theta'/\sigma_{\theta})}_{exp}/\mathrm{pdf}_{norm}$},
% axis background/.style={fill=white},
% ylabel shift = -4pt,
% xmajorgrids,
% ymajorgrids,
% yminorgrids,
% legend style={at={(1.4,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black,draw=none}
% ]
% \addplot [color=mycolor2, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor2}]
%   table[row sep=crcr]{%
% -4.39069521075637	4.8664206884064\\
% -4.34306742444763	2.23796013392579\\
% -4.2954396381389	0.88414609918375\\
% -4.24781185183017	0.682802849834665\\
% -4.20018406552144	0.985825116602566\\
% -4.1525562792127	1.70785995751355\\
% -4.10492849290397	2.35975189656657\\
% -4.05730070659524	1.75125388156099\\
% -4.00967292028651	1.88728759521962\\
% -3.96204513397778	1.59675586733237\\
% -3.91441734766904	1.58065524208255\\
% -3.86678956136031	2.10770399091219\\
% -3.81916177505158	1.57346217397241\\
% -3.77153398874285	1.3912913168666\\
% -3.72390620243411	1.63004688846648\\
% -3.67627841612538	1.97060006254852\\
% -3.62865062981665	1.92877546813837\\
% -3.58102284350792	1.82409359721261\\
% -3.53339505719918	2.10910738975679\\
% -3.48576727089045	2.10868474916597\\
% -3.43813948458172	1.83288724531802\\
% -3.39051169827299	1.71543937413641\\
% -3.34288391196426	1.82742017360357\\
% -3.29525612565552	2.0150805140029\\
% -3.24762833934679	1.88521319323863\\
% -3.20000055303806	1.89201152631668\\
% -3.15237276672933	1.77971021964523\\
% -3.10474498042059	1.69815767028111\\
% -3.05711719411186	1.70182613466115\\
% -3.00948940780313	1.63073878848081\\
% -2.9618616214944	1.65105518360809\\
% -2.91423383518567	1.60043806369384\\
% -2.86660604887693	1.49265904925476\\
% -2.8189782625682	1.47192630521524\\
% -2.77135047625947	1.45070884775941\\
% -2.72372268995074	1.49016253262184\\
% -2.676094903642	1.45733484687755\\
% -2.62846711733327	1.4019517566533\\
% -2.58083933102454	1.42277724703369\\
% -2.53321154471581	1.43663230856148\\
% -2.48558375840708	1.40348187569856\\
% -2.43795597209834	1.33839778513063\\
% -2.39032818578961	1.29428076992368\\
% -2.34270039948088	1.34020441168614\\
% -2.29507261317215	1.30120928054437\\
% -2.24744482686341	1.27034095982241\\
% -2.19981704055468	1.2666284661266\\
% -2.15218925424595	1.20436924582335\\
% -2.10456146793722	1.20632481178065\\
% -2.05693368162849	1.22308788984565\\
% -2.00930589531975	1.19686474151918\\
% -1.96167810901102	1.17247816993728\\
% -1.91405032270229	1.17973288156322\\
% -1.86642253639356	1.15892726831669\\
% -1.81879475008482	1.14075298795122\\
% -1.77116696377609	1.16182973697378\\
% -1.72353917746736	1.12727849662786\\
% -1.67591139115863	1.11686149094863\\
% -1.6282836048499	1.12625210951105\\
% -1.58065581854116	1.12160656859833\\
% -1.53302803223243	1.13137825794116\\
% -1.4854002459237	1.14002537596242\\
% -1.43777245961497	1.12355348608651\\
% -1.39014467330623	1.11747302021018\\
% -1.3425168869975	1.10544016357058\\
% -1.29488910068877	1.09789957713625\\
% -1.24726131438004	1.10143092808223\\
% -1.19963352807131	1.08316108345666\\
% -1.15200574176257	1.0680374677614\\
% -1.10437795545384	1.07715971081277\\
% -1.05675016914511	1.07597267811781\\
% -1.00912238283638	1.06812475579533\\
% -0.961494596527644	1.05549348168776\\
% -0.913866810218912	1.05440799391098\\
% -0.86623902391018	1.03099849689054\\
% -0.818611237601447	1.0150319758816\\
% -0.770983451292715	1.02452294200079\\
% -0.723355664983983	1.02313267788602\\
% -0.675727878675251	1.01192792934462\\
% -0.628100092366518	1.0019064677352\\
% -0.580472306057786	0.989524266403789\\
% -0.532844519749054	0.981217163681299\\
% -0.485216733440322	0.966551329880123\\
% -0.437588947131589	0.95534126798881\\
% -0.389961160822857	0.94749042687904\\
% -0.342333374514125	0.949954499735291\\
% -0.294705588205393	0.938088345654765\\
% -0.247077801896661	0.921620126442921\\
% -0.199450015587928	0.918035885590359\\
% -0.151822229279196	0.918144875663875\\
% -0.104194442970464	0.908659221240788\\
% -0.0565666566617314	0.90643641060278\\
% -0.0089388703529994	0.900692668092461\\
% 0.038688915955733	0.89371630122978\\
% 0.086316702264465	0.890123982671986\\
% 0.133944488573197	0.891950570407484\\
% 0.181572274881929	0.894014124405725\\
% 0.229200061190661	0.890458172704423\\
% 0.276827847499394	0.8923541490089\\
% 0.324455633808126	0.89622165408508\\
% 0.372083420116858	0.898941431132458\\
% 0.419711206425591	0.897731079829443\\
% 0.467338992734323	0.890387090508208\\
% 0.514966779043055	0.892617855465641\\
% 0.562594565351787	0.898208713325151\\
% 0.61022235166052	0.896120864568687\\
% 0.657850137969252	0.903736223252961\\
% 0.705477924277984	0.915696615383502\\
% 0.753105710586716	0.920234562220772\\
% 0.800733496895449	0.925801362537666\\
% 0.848361283204181	0.931730210629279\\
% 0.895989069512913	0.94129926260348\\
% 0.943616855821646	0.945395164816108\\
% 0.991244642130378	0.961143544415915\\
% 1.03887242843911	0.977757285427128\\
% 1.08650021474784	0.977530701202659\\
% 1.13412800105657	0.971371373105809\\
% 1.18175578736531	0.99666179885979\\
% 1.22938357367404	1.0141491455427\\
% 1.27701135998277	1.02071788199931\\
% 1.3246391462915	1.0150575195351\\
% 1.37226693260024	1.02122550649487\\
% 1.41989471890897	1.05177486053015\\
% 1.4675225052177	1.08451710803855\\
% 1.51515029152643	1.09990588591286\\
% 1.56277807783516	1.1173598594158\\
% 1.6104058641439	1.12235378816136\\
% 1.65803365045263	1.12067132754646\\
% 1.70566143676136	1.15318438645829\\
% 1.75328922307009	1.16016898387862\\
% 1.80091700937883	1.18945570713626\\
% 1.84854479568756	1.24239967350391\\
% 1.89617258199629	1.27064602754014\\
% 1.94380036830502	1.29632813274509\\
% 1.99142815461375	1.32558239960043\\
% 2.03905594092249	1.3492420466971\\
% 2.08668372723122	1.38493110352474\\
% 2.13431151353995	1.45202878477453\\
% 2.18193929984868	1.44764278473031\\
% 2.22956708615742	1.47816981883359\\
% 2.27719487246615	1.51226102235748\\
% 2.32482265877488	1.54351211047798\\
% 2.37245044508361	1.61784860088147\\
% 2.42007823139235	1.71185575900779\\
% 2.46770601770108	1.78511768785488\\
% 2.51533380400981	1.81157624174853\\
% 2.56296159031854	1.85201232972524\\
% 2.61058937662727	1.84789942532131\\
% 2.65821716293601	1.99504433853614\\
% 2.70584494924474	1.97598746873146\\
% 2.75347273555347	2.08123315262082\\
% 2.8011005218622	2.23000586404703\\
% 2.84872830817093	2.26576519618384\\
% 2.89635609447967	2.38558657752122\\
% 2.9439838807884	2.60523966821174\\
% 2.99161166709713	2.77538996634897\\
% 3.03923945340586	2.65119661575113\\
% 3.0868672397146	2.56845404206886\\
% 3.13449502602333	2.90992647104435\\
% 3.18212281233206	3.30971527288641\\
% 3.22975059864079	3.47733777238359\\
% 3.27737838494953	3.36586432700056\\
% 3.32500617125826	3.53869364953475\\
% 3.37263395756699	3.9983885741044\\
% 3.42026174387572	4.24845038406425\\
% 3.46788953018445	4.2391378628796\\
% 3.51551731649319	4.60896817627702\\
% 3.56314510280192	4.82846590338005\\
% 3.61077288911065	4.6483395620138\\
% 3.65840067541938	4.93024152553921\\
% 3.70602846172812	5.57740537218249\\
% 3.75365624803685	5.52298693496769\\
% 3.80128403434558	5.11857484090036\\
% 3.84891182065431	5.71764487726564\\
% 3.89653960696304	5.99918243011348\\
% 3.94416739327178	6.04177267181511\\
% 3.99179517958051	5.96409388418776\\
% 4.03942296588924	6.6395953377271\\
% 4.08705075219797	8.4967181732616\\
% 4.13467853850671	9.52200558444528\\
% 4.18230632481544	8.66395196037067\\
% 4.22993411112417	7.31250502593733\\
% 4.2775618974329	10.2058720597761\\
% 4.32518968374163	8.37687655437026\\
% 4.37281747005037	10.3644968144254\\
% 4.4204452563591	12.325025273382\\
% 4.46807304266783	17.9769749290983\\
% 4.51570082897656	11.3342113760262\\
% 4.56332861528529	8.41567499121726\\
% 4.61095640159403	9.2122266601358\\
% 4.65858418790276	4.40170315840666\\
% 4.70621197421149	12.6480063633441\\
% 4.75383976052022	18.1576733217085\\
% 4.80146754682896	19.307091261041\\
% 4.84909533313769	9.82415377791285\\
% 4.89672311944642	1.53163326057062\\
% 4.94435090575515	0\\
% 4.99197869206389	0\\
% 5.03960647837262	20.3385527872252\\
% 5.08723426468135	97.8448396556348\\
% };
% \addlegendentry{$\text{u'/}\sigma{}_\text{u}$}

% \addplot [color=mycolor1, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor1}]
%   table[row sep=crcr]{%
% -4.65891264028589	15.6493637185169\\
% -4.61176778719693	4.52608763180296\\
% -4.56462293410797	6.15597520025579\\
% -4.51747808101902	5.76217006972365\\
% -4.47033322793006	4.93294180198555\\
% -4.42318837484111	12.3156531387154\\
% -4.37604352175215	7.48807852395771\\
% -4.3288986686632	5.83053608635242\\
% -4.28175381557424	5.51985646543939\\
% -4.23460896248528	5.98960855705225\\
% -4.18746410939633	6.20486486635459\\
% -4.14031925630737	6.79639389627035\\
% -4.09317440321842	6.66748471909114\\
% -4.04602955012946	4.84572294354371\\
% -3.99888469704051	3.62329992805698\\
% -3.95173984395155	5.08937568793846\\
% -3.9045949908626	5.89700585781599\\
% -3.85745013777364	5.61590968929254\\
% -3.81030528468468	4.80490829928088\\
% -3.76316043159573	4.70272614751019\\
% -3.71601557850677	5.41347613068532\\
% -3.66887072541782	4.60793473674264\\
% -3.62172587232886	4.96855722094634\\
% -3.57458101923991	5.25527908715587\\
% -3.52743616615095	4.7960528837042\\
% -3.480291313062	4.64799639168047\\
% -3.43314645997304	4.68661963823481\\
% -3.38600160688408	4.31027218991714\\
% -3.33885675379513	3.95410649711853\\
% -3.29171190070617	3.87712834093609\\
% -3.24456704761722	3.69061500438663\\
% -3.19742219452826	3.32851838255591\\
% -3.15027734143931	3.47254530632254\\
% -3.10313248835035	3.36790928093801\\
% -3.05598763526139	3.34060879590417\\
% -3.00884278217244	3.39749711690195\\
% -2.96169792908348	2.96875378275355\\
% -2.91455307599453	3.02064376861609\\
% -2.86740822290557	2.78105170117853\\
% -2.82026336981662	2.61051741894824\\
% -2.77311851672766	2.7702385014077\\
% -2.72597366363871	2.69915936251575\\
% -2.67882881054975	2.64725594833568\\
% -2.63168395746079	2.63508279909224\\
% -2.58453910437184	2.54563408477132\\
% -2.53739425128288	2.46009921223917\\
% -2.49024939819393	2.32775537550988\\
% -2.44310454510497	2.23239092811152\\
% -2.39595969201602	2.23389622830254\\
% -2.34881483892706	2.14373481729905\\
% -2.3016699858381	2.11179226095421\\
% -2.25452513274915	2.05066287436208\\
% -2.20738027966019	1.97000292531143\\
% -2.16023542657124	1.90324392821774\\
% -2.11309057348228	1.87823820920728\\
% -2.06594572039333	1.82681940656791\\
% -2.01880086730437	1.76266535283199\\
% -1.97165601421542	1.7292879810705\\
% -1.92451116112646	1.66308927189958\\
% -1.8773663080375	1.6030398461525\\
% -1.83022145494855	1.56679481790019\\
% -1.78307660185959	1.54137403273257\\
% -1.73593174877064	1.49638800723781\\
% -1.68878689568168	1.44355097832683\\
% -1.64164204259273	1.39658089269466\\
% -1.59449718950377	1.33692623606906\\
% -1.54735233641482	1.31173354288463\\
% -1.50020748332586	1.27339287161864\\
% -1.4530626302369	1.24015089243381\\
% -1.40591777714795	1.2024375472035\\
% -1.35877292405899	1.1560625795384\\
% -1.31162807097004	1.12558524904768\\
% -1.26448321788108	1.12159390607524\\
% -1.21733836479213	1.08321895724439\\
% -1.17019351170317	1.06416552356826\\
% -1.12304865861421	1.02918075129672\\
% -1.07590380552526	1.01113199010916\\
% -1.0287589524363	0.993144282727369\\
% -0.981614099347348	0.980269298210478\\
% -0.934469246258392	0.959826393944399\\
% -0.887324393169437	0.952936021496826\\
% -0.840179540080481	0.943689811799999\\
% -0.793034686991525	0.935709396558863\\
% -0.74588983390257	0.916014314430531\\
% -0.698744980813614	0.897706173365232\\
% -0.651600127724659	0.901558056514313\\
% -0.604455274635703	0.896283246307555\\
% -0.557310421546747	0.885070089024194\\
% -0.510165568457792	0.877402687059909\\
% -0.463020715368836	0.876340627201606\\
% -0.415875862279881	0.881178061704802\\
% -0.368731009190925	0.88574074927123\\
% -0.321586156101969	0.875493530770296\\
% -0.274441303013014	0.875199658010558\\
% -0.227296449924058	0.868287531660324\\
% -0.180151596835102	0.871508267840501\\
% -0.133006743746147	0.868950889512225\\
% -0.0858618906571912	0.862025445489704\\
% -0.0387170375682358	0.868523638098454\\
% 0.00842781552072008	0.871138882815561\\
% 0.0555726686096756	0.872827276809879\\
% 0.102717521698631	0.870537093019286\\
% 0.149862374787587	0.877695518833032\\
% 0.197007227876543	0.885454270341804\\
% 0.244152080965498	0.879158118046363\\
% 0.291296934054454	0.890336737870403\\
% 0.338441787143409	0.88429700732066\\
% 0.385586640232365	0.89418318587943\\
% 0.432731493321321	0.903936552924624\\
% 0.479876346410276	0.910438277816075\\
% 0.527021199499232	0.919619676697098\\
% 0.574166052588188	0.934949431483268\\
% 0.621310905677143	0.942848106904353\\
% 0.668455758766099	0.953283698699044\\
% 0.715600611855054	0.94937047973822\\
% 0.76274546494401	0.942939292538229\\
% 0.809890318032966	0.955126857749635\\
% 0.857035171121921	0.971441300626737\\
% 0.904180024210877	0.982812595390276\\
% 0.951324877299832	1.00166533630786\\
% 0.998469730388788	1.0093090006131\\
% 1.04561458347774	1.01120056817746\\
% 1.0927594365667	1.01909677282499\\
% 1.13990428965565	1.0372566915418\\
% 1.18704914274461	1.04726641910784\\
% 1.23419399583357	1.04142116256359\\
% 1.28133884892252	1.0644079007036\\
% 1.32848370201148	1.10096367447684\\
% 1.37562855510043	1.11082513122083\\
% 1.42277340818939	1.11651420530381\\
% 1.46991826127834	1.13631917643581\\
% 1.5170631143673	1.14558173977093\\
% 1.56420796745626	1.1784765099052\\
% 1.61135282054521	1.18931312514035\\
% 1.65849767363417	1.18508824027509\\
% 1.70564252672312	1.21181631578746\\
% 1.75278737981208	1.23268587260112\\
% 1.79993223290103	1.2560431418093\\
% 1.84707708598999	1.28808453832409\\
% 1.89422193907894	1.27596205211733\\
% 1.9413667921679	1.29384704399476\\
% 1.98851164525686	1.32963694496835\\
% 2.03565649834581	1.37856421104478\\
% 2.08280135143477	1.3895341716084\\
% 2.12994620452372	1.41354713205848\\
% 2.17709105761268	1.45944380884683\\
% 2.22423591070163	1.46483539807387\\
% 2.27138076379059	1.45243894807265\\
% 2.31852561687954	1.5130037873836\\
% 2.3656704699685	1.51205866671463\\
% 2.41281532305746	1.5709087423252\\
% 2.45996017614641	1.60705224972303\\
% 2.50710502923537	1.69448614960026\\
% 2.55424988232432	1.74401853019693\\
% 2.60139473541328	1.83641287305376\\
% 2.64853958850223	1.91356668872837\\
% 2.69568444159119	1.9713619030993\\
% 2.74282929468015	2.0261208551739\\
% 2.7899741477691	2.06566316256956\\
% 2.83711900085806	2.18788520025677\\
% 2.88426385394701	2.25501230204998\\
% 2.93140870703597	2.33641752777333\\
% 2.97855356012492	2.5734686091309\\
% 3.02569841321388	2.48108468681031\\
% 3.07284326630283	2.51172413528935\\
% 3.11998811939179	2.78499026004779\\
% 3.16713297248075	2.86488673591969\\
% 3.2142778255697	2.97394697651467\\
% 3.26142267865866	3.20904272795035\\
% 3.30856753174761	3.15724625204996\\
% 3.35571238483657	3.21351796554514\\
% 3.40285723792552	3.29910143445587\\
% 3.45000209101448	3.31296571411201\\
% 3.49714694410344	3.47820014180935\\
% 3.54429179719239	3.89358278547087\\
% 3.59143665028135	4.85228341894763\\
% 3.6385815033703	5.06929008910668\\
% 3.68572635645926	4.63848472504926\\
% 3.73287120954821	5.31714635080568\\
% 3.78001606263717	5.29474352950143\\
% 3.82716091572612	5.41384276298549\\
% 3.87430576881508	5.62363480227984\\
% 3.92145062190404	4.69319276314299\\
% 3.96859547499299	5.19707910181433\\
% 4.01574032808195	6.57696529469461\\
% 4.0628851811709	7.21960471527531\\
% 4.11003003425986	6.51685423833685\\
% 4.15717488734881	8.21126478700659\\
% 4.20431974043777	9.48170459937625\\
% 4.25146459352673	8.86968914577587\\
% 4.29860944661568	7.47793755144391\\
% 4.34575429970464	10.6801956568971\\
% 4.39289915279359	13.2640371520861\\
% 4.44004400588255	11.6087800121257\\
% 4.4871888589715	12.4347171991675\\
% 4.53433371206046	20.4791293835261\\
% 4.58147856514941	18.192853210662\\
% 4.62862341823837	11.6144957872029\\
% 4.67576827132733	12.630854684133\\
% 4.72291312441628	27.8440702464942\\
% };
% \addlegendentry{$\theta\text{'/}\sigma{}_\theta$}


% \addplot [color=mycolor3, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor3},forget plot]
%   table[row sep=crcr]{%
% -4.02029280022338	1.24150484063745\\
% -3.97687440003228	0.350335387428369\\
% -3.93345599984118	0.447367403775875\\
% -3.89003759965008	0.488360252268205\\
% -3.84661919945897	0.458336900731874\\
% -3.80320079926787	0.278204290599367\\
% -3.75978239907677	0.344229525206817\\
% -3.71636399888566	0.629811546362177\\
% -3.67294559869456	0.632448667771804\\
% -3.62952719850346	0.615333436209809\\
% -3.58610879831235	0.546385287682137\\
% -3.54269039812125	0.492625261744652\\
% -3.49927199793015	0.545744538707776\\
% -3.45585359773905	0.648234453018204\\
% -3.41243519754794	0.792438606579526\\
% -3.36901679735684	0.810220711338479\\
% -3.32559839716574	0.853982595493025\\
% -3.28217999697463	0.869722001700905\\
% -3.23876159678353	0.862122104015613\\
% -3.19534319659243	0.86724824040893\\
% -3.15192479640132	0.915540588143672\\
% -3.10850639621022	0.939827197445304\\
% -3.06508799601912	0.987040522647391\\
% -3.02166959582801	1.03116837983026\\
% -2.97825119563691	1.02681281315443\\
% -2.93483279544581	1.02422028303056\\
% -2.89141439525471	1.12218339579472\\
% -2.8479959950636	1.21153286109154\\
% -2.8045775948725	1.11994892854621\\
% -2.7611591946814	1.11230311803407\\
% -2.71774079449029	1.14133831155519\\
% -2.67432239429919	1.14610750618597\\
% -2.63090399410809	1.13561185085062\\
% -2.58748559391698	1.10880210291028\\
% -2.54406719372588	1.1076537023042\\
% -2.50064879353478	1.13424039715147\\
% -2.45723039334367	1.12098904422696\\
% -2.41381199315257	1.06198020357742\\
% -2.37039359296147	1.11252550184996\\
% -2.32697519277037	1.10587860191171\\
% -2.28355679257926	1.14751297371026\\
% -2.24013839238816	1.13200601814129\\
% -2.19671999219706	1.09734202672404\\
% -2.15330159200595	1.08877024108604\\
% -2.10988319181485	1.09843900378273\\
% -2.06646479162375	1.08358641755863\\
% -2.02304639143264	1.09287220431508\\
% -1.97962799124154	1.09476548079612\\
% -1.93620959105044	1.11766383660004\\
% -1.89279119085933	1.11329016185389\\
% -1.84937279066823	1.07965263107604\\
% -1.80595439047713	1.06201580641781\\
% -1.76253599028603	1.06802258039507\\
% -1.71911759009492	1.07441714990311\\
% -1.67569918990382	1.07352684085775\\
% -1.63228078971272	1.07307822090976\\
% -1.58886238952161	1.06285704434639\\
% -1.54544398933051	1.04986301114837\\
% -1.50202558913941	1.04661556252603\\
% -1.4586071889483	1.04405790091044\\
% -1.4151887887572	1.0322827438719\\
% -1.3717703885661	1.03193531795562\\
% -1.328351988375	1.03006153822267\\
% -1.28493358818389	1.03210108965689\\
% -1.24151518799279	1.0254706876566\\
% -1.19809678780169	1.02779997109685\\
% -1.15467838761058	1.02050844910799\\
% -1.11125998741948	1.00400179530824\\
% -1.06784158722838	0.993701810522813\\
% -1.02442318703727	1.00517052588074\\
% -0.98100478684617	1.00517891437214\\
% -0.937586386655067	1.00419404314221\\
% -0.894167986463964	0.999847999304847\\
% -0.850749586272861	1.00586552572845\\
% -0.807331186081758	1.0086130946513\\
% -0.763912785890655	0.993903016834918\\
% -0.720494385699552	0.986403379360377\\
% -0.677075985508449	0.986354614027381\\
% -0.633657585317346	0.985361043746002\\
% -0.590239185126243	0.97997598399714\\
% -0.54682078493514	0.983546373133303\\
% -0.503402384744037	0.970306602598333\\
% -0.459983984552933	0.967471059746723\\
% -0.41656558436183	0.981990591326556\\
% -0.373147184170727	0.989577765154901\\
% -0.329728783979624	0.974611652728294\\
% -0.286310383788521	0.966903414726825\\
% -0.242891983597418	0.984102646252472\\
% -0.199473583406315	0.986818186864795\\
% -0.156055183215212	0.971607062308246\\
% -0.112636783024109	0.972267266425847\\
% -0.0692183828330057	0.963245881399919\\
% -0.0257999826419024	0.96974491526712\\
% 0.0176184175492003	0.973221693828618\\
% 0.0610368177403033	0.964905733568174\\
% 0.104455217931407	0.965938052677435\\
% 0.14787361812251	0.960847305431317\\
% 0.191292018313613	0.965951647590317\\
% 0.234710418504716	0.97021987526091\\
% 0.278128818695819	0.964177054012828\\
% 0.321547218886922	0.964397484533543\\
% 0.364965619078025	0.969139606993595\\
% 0.408384019269128	0.976303755059496\\
% 0.451802419460231	0.98568111198234\\
% 0.495220819651334	0.985663865823847\\
% 0.538639219842437	0.985071950688628\\
% 0.582057620033541	0.981682079968776\\
% 0.625476020224643	0.972164496701877\\
% 0.668894420415746	0.975194454873839\\
% 0.71231282060685	0.974578250112613\\
% 0.755731220797953	0.96987806547078\\
% 0.799149620989056	0.972710020592657\\
% 0.842568021180159	0.972307010768925\\
% 0.885986421371262	0.983610720959341\\
% 0.929404821562365	0.98827183727488\\
% 0.972823221753468	0.98322245112372\\
% 1.01624162194457	0.992311929372483\\
% 1.05966002213567	0.995889674110928\\
% 1.10307842232678	0.994877974340514\\
% 1.14649682251788	0.988357619070194\\
% 1.18991522270898	0.991037714511377\\
% 1.23333362290009	0.996396745258182\\
% 1.27675202309119	0.994610268013095\\
% 1.32017042328229	1.00001106339331\\
% 1.3635888234734	0.998048518094718\\
% 1.4070072236645	1.00589418133046\\
% 1.4504256238556	1.00380024365538\\
% 1.49384402404671	1.01879827367433\\
% 1.53726242423781	1.02108916737011\\
% 1.58068082442891	1.00656623617291\\
% 1.62409922462001	1.00179118413672\\
% 1.66751762481112	1.01959409919452\\
% 1.71093602500222	1.04345944761309\\
% 1.75435442519332	1.04409921996373\\
% 1.79777282538443	1.07989988084049\\
% 1.84119122557553	1.07933054029004\\
% 1.88460962576663	1.07904995353667\\
% 1.92802802595774	1.11292507935232\\
% 1.97144642614884	1.11392216287114\\
% 2.01486482633994	1.10504660715487\\
% 2.05828322653104	1.14084416836161\\
% 2.10170162672215	1.14068639286384\\
% 2.14512002691325	1.19211698497447\\
% 2.18853842710435	1.20090061788986\\
% 2.23195682729546	1.206864871171\\
% 2.27537522748656	1.24314127314544\\
% 2.31879362767766	1.24930433726582\\
% 2.36221202786877	1.27774490759374\\
% 2.40563042805987	1.3208190327007\\
% 2.44904882825097	1.28276473937581\\
% 2.49246722844208	1.30980417961142\\
% 2.53588562863318	1.3159139680252\\
% 2.57930402882428	1.34487757829688\\
% 2.62272242901538	1.31575634449779\\
% 2.66614082920649	1.34235504997271\\
% 2.70955922939759	1.40185500548597\\
% 2.75297762958869	1.38670289285701\\
% 2.7963960297798	1.35476862396713\\
% 2.8398144299709	1.45381339226138\\
% 2.883232830162	1.50355265518919\\
% 2.92665123035311	1.48989694124178\\
% 2.97006963054421	1.55392950261694\\
% 3.01348803073531	1.62422368253585\\
% 3.05690643092642	1.66761684763421\\
% 3.10032483111752	1.5640359082853\\
% 3.14374323130862	1.71900541123243\\
% 3.18716163149972	1.82056041475194\\
% 3.23058003169083	1.87728868020905\\
% 3.27399843188193	1.89156519728821\\
% 3.31741683207303	1.88053083166983\\
% 3.36083523226414	1.70924533265117\\
% 3.40425363245524	2.04453174240549\\
% 3.44767203264634	1.90984603192278\\
% 3.49109043283745	2.05517936669963\\
% 3.53450883302855	2.08592215984493\\
% 3.57792723321965	1.97087828318097\\
% 3.62134563341076	2.00470464283358\\
% 3.66476403360186	2.10779274546864\\
% 3.70818243379296	1.94540836482294\\
% 3.75160083398406	1.83758801479053\\
% 3.79501923417517	2.04754634486467\\
% 3.83843763436627	2.08300369451607\\
% 3.88185603455737	2.4806905383492\\
% 3.92527443474848	2.5170689512722\\
% 3.96869283493958	3.3504676710664\\
% 4.01211123513068	2.82039711372905\\
% 4.05552963532179	2.28698248011355\\
% 4.09894803551289	2.66845561495929\\
% 4.14236643570399	3.47807273804699\\
% 4.1857848358951	3.51957038768943\\
% 4.2292032360862	4.31522417123272\\
% 4.2726216362773	3.54174613586398\\
% 4.3160400364684	4.20761384205655\\
% 4.35945843665951	5.35074026902701\\
% 4.40287683685061	9.04614093988916\\
% 4.44629523704171	7.69700235063016\\
% 4.48971363723282	4.28957430082152\\
% 4.53313203742392	2.69765966695077\\
% 4.57655043761502	4.60273822914904\\
% 4.61996883780613	11.6457796597644\\
% };


% \addplot [color=mycolor4, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor4}, forget plot]
%   table[row sep=crcr]{%
% -4.04518965615418	1.33899683810615\\
% -3.99746426648285	0.54744865154561\\
% -3.94973887681151	0.169579207049623\\
% -3.90201348714018	0.454508802665379\\
% -3.85428809746885	0.463206280777494\\
% -3.80656270779752	0.595919169161514\\
% -3.75883731812618	0.43173342844369\\
% -3.71111192845485	0.478725088329991\\
% -3.66338653878352	0.626331726608728\\
% -3.61566114911218	0.971153801546105\\
% -3.56793575944085	0.854148819908763\\
% -3.52021036976952	0.631780664910649\\
% -3.47248498009818	0.58067450186139\\
% -3.42475959042685	0.744308408207667\\
% -3.37703420075552	0.680408426704196\\
% -3.32930881108419	0.647606231464743\\
% -3.28158342141285	0.675353873184975\\
% -3.23385803174152	0.657514892520329\\
% -3.18613264207019	0.733791899437038\\
% -3.13840725239885	0.778644692873976\\
% -3.09068186272752	0.759052021367531\\
% -3.04295647305619	0.72112529655722\\
% -2.99523108338485	0.619432292312034\\
% -2.94750569371352	0.636910347734444\\
% -2.89978030404219	0.682982134128949\\
% -2.85205491437086	0.687353977326754\\
% -2.80432952469952	0.713210534434708\\
% -2.75660413502819	0.690786460025102\\
% -2.70887874535686	0.749266285776037\\
% -2.66115335568552	0.730896177196551\\
% -2.61342796601419	0.776006440462986\\
% -2.56570257634286	0.785455698568893\\
% -2.51797718667152	0.822891948268602\\
% -2.47025179700019	0.82228893895618\\
% -2.42252640732886	0.855457927193357\\
% -2.37480101765752	0.837043174903278\\
% -2.32707562798619	0.847408271780533\\
% -2.27935023831486	0.864736510723334\\
% -2.23162484864353	0.847817787411317\\
% -2.18389945897219	0.852256233097154\\
% -2.13617406930086	0.894095027199099\\
% -2.08844867962953	0.931115962051764\\
% -2.04072328995819	0.968980581164496\\
% -1.99299790028686	0.945057837812232\\
% -1.94527251061553	0.940837415243576\\
% -1.89754712094419	0.963451440452263\\
% -1.84982173127286	0.966917351361614\\
% -1.80209634160153	0.998860627217255\\
% -1.7543709519302	0.98869893467253\\
% -1.70664556225886	0.992118642926732\\
% -1.65892017258753	0.991780462695351\\
% -1.6111947829162	1.01693637986527\\
% -1.56346939324486	1.04034823688266\\
% -1.51574400357353	1.02915507525699\\
% -1.4680186139022	1.02346763536452\\
% -1.42029322423086	1.0403680291578\\
% -1.37256783455953	1.04623065899861\\
% -1.3248424448882	1.04342487422116\\
% -1.27711705521686	1.05737073729508\\
% -1.22939166554553	1.06269225370322\\
% -1.1816662758742	1.04844227035766\\
% -1.13394088620287	1.04909563755324\\
% -1.08621549653153	1.04749007181562\\
% -1.0384901068602	1.04388132165809\\
% -0.990764717188867	1.04940581167364\\
% -0.943039327517534	1.04256475084395\\
% -0.895313937846201	1.04675541121491\\
% -0.847588548174868	1.04321253479308\\
% -0.799863158503535	1.04552412442363\\
% -0.752137768832201	1.04999702491747\\
% -0.704412379160869	1.05655222273774\\
% -0.656686989489535	1.05188006522465\\
% -0.608961599818203	1.04574087865482\\
% -0.561236210146869	1.04260021113627\\
% -0.513510820475536	1.04334975451777\\
% -0.465785430804203	1.04464372654196\\
% -0.41806004113287	1.03963913323206\\
% -0.370334651461537	1.039262862526\\
% -0.322609261790204	1.02780265173094\\
% -0.274883872118871	1.01740986103756\\
% -0.227158482447538	1.01960409310366\\
% -0.179433092776205	1.0299802385078\\
% -0.131707703104872	1.02514130307975\\
% -0.0839823134335389	1.01168750679978\\
% -0.0362569237622061	1.00049551495692\\
% 0.0114684659091272	1.00379620853047\\
% 0.0591938555804602	0.992171718081978\\
% 0.106919245251793	0.99345659087955\\
% 0.154644634923126	0.993136882135712\\
% 0.202370024594459	0.99543761100079\\
% 0.250095414265792	0.993065978492403\\
% 0.297820803937125	0.975638981989618\\
% 0.345546193608458	0.979467612436256\\
% 0.393271583279792	0.969245668410569\\
% 0.440996972951125	0.969594593567776\\
% 0.488722362622458	0.964702380312142\\
% 0.536447752293791	0.969554873208208\\
% 0.584173141965124	0.96059426561864\\
% 0.631898531636457	0.958749922326045\\
% 0.67962392130779	0.957423248465045\\
% 0.727349310979123	0.948472348257524\\
% 0.775074700650456	0.940095264335015\\
% 0.822800090321789	0.94374444072323\\
% 0.870525479993122	0.944774579093508\\
% 0.918250869664455	0.936916683291806\\
% 0.965976259335788	0.931976775433008\\
% 1.01370164900712	0.933549443685117\\
% 1.06142703867845	0.928683285551091\\
% 1.10915242834979	0.922143746921177\\
% 1.15687781802112	0.927786620849644\\
% 1.20460320769245	0.926598728790848\\
% 1.25232859736379	0.914506804773131\\
% 1.30005398703512	0.921825202624152\\
% 1.34777937670645	0.937893665156176\\
% 1.39550476637779	0.939483162492325\\
% 1.44323015604912	0.936008227208557\\
% 1.49095554572045	0.940263005480199\\
% 1.53868093539178	0.954807667767239\\
% 1.58640632506312	0.968994202593298\\
% 1.63413171473445	0.956890284126314\\
% 1.68185710440578	0.92623678381433\\
% 1.72958249407712	0.953129170785173\\
% 1.77730788374845	0.988692561929129\\
% 1.82503327341978	0.997935703170742\\
% 1.87275866309112	1.00120231325523\\
% 1.92048405276245	1.00316069551315\\
% 1.96820944243378	1.02483111181154\\
% 2.01593483210511	1.02415339342809\\
% 2.06366022177645	1.02184655933824\\
% 2.11138561144778	1.04694004854736\\
% 2.15911100111911	1.08584754652249\\
% 2.20683639079045	1.08584550564329\\
% 2.25456178046178	1.09384688942108\\
% 2.30228717013311	1.11019563115321\\
% 2.35001255980445	1.12872156355654\\
% 2.39773794947578	1.14889877397515\\
% 2.44546333914711	1.20204924099089\\
% 2.49318872881845	1.24226330976417\\
% 2.54091411848978	1.29216239315096\\
% 2.58863950816111	1.2752842362405\\
% 2.63636489783244	1.35294123411359\\
% 2.68409028750378	1.45921853817683\\
% 2.73181567717511	1.39547813710458\\
% 2.77954106684644	1.49810149033925\\
% 2.82726645651778	1.62460647316422\\
% 2.87499184618911	1.61713941037295\\
% 2.92271723586044	1.74646664939997\\
% 2.97044262553178	1.82046916657645\\
% 3.01816801520311	1.97204876073059\\
% 3.06589340487444	2.01943452543922\\
% 3.11361879454577	2.03526634726849\\
% 3.16134418421711	2.10154558107758\\
% 3.20906957388844	2.20235671154665\\
% 3.25679496355977	2.34117150213211\\
% 3.30452035323111	2.4170547255994\\
% 3.35224574290244	2.56320003181532\\
% 3.39997113257377	2.64651822614021\\
% 3.44769652224511	3.05148947819652\\
% 3.49542191191644	3.30525976955377\\
% 3.54314730158777	3.2801623836428\\
% 3.5908726912591	3.96880340514527\\
% 3.63859808093044	3.79813922575274\\
% 3.68632347060177	3.93670336312359\\
% 3.7340488602731	3.49005741727553\\
% 3.78177424994444	4.07582475849087\\
% 3.82949963961577	4.43234154999775\\
% 3.8772250292871	5.28543303644628\\
% 3.92495041895844	5.88917608554547\\
% 3.97267580862977	6.00753863423161\\
% 4.0204011983011	6.38859170629829\\
% 4.06812658797244	7.36926751423228\\
% 4.11585197764377	5.18724635303876\\
% 4.1635773673151	6.82214288333404\\
% 4.21130275698643	8.74661439857402\\
% 4.25902814665777	10.6218260008029\\
% 4.3067535363291	8.12529943465146\\
% 4.35447892600043	9.08880935424959\\
% 4.40220431567177	13.0324641104986\\
% 4.4499297053431	15.6938723209118\\
% 4.49765509501443	12.4005552700241\\
% 4.54538048468577	13.9582075268564\\
% 4.5931058743571	17.539508894259\\
% 4.64083126402843	19.6953719493523\\
% 4.68855665369977	34.6263480415164\\
% 4.7362820433711	22.8581534430249\\
% 4.78400743304243	9.64723549465872\\
% 4.83173282271376	10.5069431462649\\
% 4.8794582123851	22.6598658075827\\
% 4.92718360205643	36.9743407944086\\
% 4.97490899172776	44.7480553395137\\
% 5.0226343813991	64.6728993114211\\
% 5.07035977107043	20.6910527181257\\
% 5.11808516074176	31.761020971945\\
% 5.1658105504131	56.3762152620354\\
% 5.21353594008443	98.7493884877112\\
% 5.26126132975576	85.9246752088672\\
% 5.30898671942709	77.153773734947\\
% 5.35671210909843	16.1158255973481\\
% 5.40443749876976	138.408108185943\\
% 5.45216288844109	665.85461090425\\
% };

% \addplot [color=mycolor5, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor5}, forget plot]
%   table[row sep=crcr]{%
% -4.36755971515259	4.38292135680342\\
% -4.3212490572506	2.05270191347054\\
% -4.27493839934862	1.53907820191235\\
% -4.22862774144664	1.98448834894408\\
% -4.18231708354465	1.08454234950661\\
% -4.13600642564267	0.84828332090653\\
% -4.08969576774068	1.0411683398288\\
% -4.0433851098387	1.14356751099417\\
% -3.99707445193671	0.773486149139089\\
% -3.95076379403473	1.19811154366336\\
% -3.90445313613274	1.07354848090665\\
% -3.85814247823076	1.25441881883365\\
% -3.81183182032877	1.45892850065407\\
% -3.76552116242679	1.96624374620708\\
% -3.7192105045248	2.05458732974027\\
% -3.67289984662282	2.46143378553334\\
% -3.62658918872083	2.52583086752403\\
% -3.58027853081885	2.37815479691167\\
% -3.53396787291686	2.08925260154448\\
% -3.48765721501488	2.14425389423221\\
% -3.44134655711289	2.2783786679666\\
% -3.39503589921091	2.39573060941747\\
% -3.34872524130892	2.56061890759844\\
% -3.30241458340694	2.38891165079013\\
% -3.25610392550495	2.29002146341544\\
% -3.20979326760297	2.31539521429936\\
% -3.16348260970098	2.57386698681198\\
% -3.117171951799	2.37437898941261\\
% -3.07086129389702	2.4365537163399\\
% -3.02455063599503	2.37248037089985\\
% -2.97823997809305	2.28332284571689\\
% -2.93192932019106	2.19567321634205\\
% -2.88561866228908	2.18214413755737\\
% -2.83930800438709	2.28019078507598\\
% -2.79299734648511	2.23423967866633\\
% -2.74668668858312	2.08742782665571\\
% -2.70037603068114	1.98924962631816\\
% -2.65406537277915	2.02873051692911\\
% -2.60775471487717	2.0108207609594\\
% -2.56144405697518	2.02866950305461\\
% -2.5151333990732	1.96312827163359\\
% -2.46882274117121	1.84482567093839\\
% -2.42251208326923	1.76692253732904\\
% -2.37620142536724	1.77677875284633\\
% -2.32989076746526	1.75009436204011\\
% -2.28358010956327	1.71146308860025\\
% -2.23726945166129	1.61483892316087\\
% -2.1909587937593	1.5639131864091\\
% -2.14464813585732	1.59193151514132\\
% -2.09833747795533	1.52907713112264\\
% -2.05202682005335	1.47806999259993\\
% -2.00571616215136	1.43485470755267\\
% -1.95940550424938	1.41003073671819\\
% -1.91309484634739	1.34741726165301\\
% -1.86678418844541	1.36749688903108\\
% -1.82047353054342	1.34224494484053\\
% -1.77416287264144	1.25831480645926\\
% -1.72785221473946	1.26635788418913\\
% -1.68154155683747	1.26345797070161\\
% -1.63523089893549	1.24104819295816\\
% -1.5889202410335	1.1958216863083\\
% -1.54260958313152	1.17512755186209\\
% -1.49629892522953	1.16221353329279\\
% -1.44998826732755	1.15343356860639\\
% -1.40367760942556	1.13117300132339\\
% -1.35736695152358	1.09960772046864\\
% -1.31105629362159	1.082652953741\\
% -1.26474563571961	1.0745739523156\\
% -1.21843497781762	1.07398821840241\\
% -1.17212431991564	1.04053109640938\\
% -1.12581366201365	1.01981898662068\\
% -1.07950300411167	1.01295470709958\\
% -1.03319234620968	0.998154719121442\\
% -0.986881688307699	0.991854653421188\\
% -0.940571030405714	0.980285410418573\\
% -0.894260372503729	0.973335041502275\\
% -0.847949714601744	0.965681639599089\\
% -0.801639056699759	0.955511586379676\\
% -0.755328398797774	0.958218760216542\\
% -0.70901774089579	0.965053469067445\\
% -0.662707082993805	0.936263048184057\\
% -0.61639642509182	0.925637919840285\\
% -0.570085767189835	0.930124938116723\\
% -0.523775109287851	0.924398756014882\\
% -0.477464451385866	0.929691103736543\\
% -0.431153793483881	0.930477900746458\\
% -0.384843135581896	0.930384871143981\\
% -0.338532477679911	0.921556687052239\\
% -0.292221819777926	0.922219699406555\\
% -0.245911161875942	0.905352484828965\\
% -0.199600503973957	0.911682421628324\\
% -0.153289846071972	0.926955836475942\\
% -0.106979188169987	0.915284012041628\\
% -0.0606685302680023	0.909307834093679\\
% -0.0143578723660176	0.916088905297619\\
% 0.031952785535967	0.917138370290224\\
% 0.0782634434379516	0.91699826369701\\
% 0.124574101339937	0.920862076382901\\
% 0.170884759241921	0.918798790706024\\
% 0.217195417143906	0.927114465961636\\
% 0.263506075045891	0.928275825291508\\
% 0.309816732947876	0.92499320992186\\
% 0.356127390849861	0.934189488639237\\
% 0.402438048751846	0.933653760072264\\
% 0.44874870665383	0.938769911435051\\
% 0.495059364555815	0.939022101200606\\
% 0.5413700224578	0.953695240396581\\
% 0.587680680359785	0.956744020271937\\
% 0.63399133826177	0.964164883795553\\
% 0.680301996163754	0.963026573213555\\
% 0.726612654065739	0.965364791915446\\
% 0.772923311967724	0.964024467283251\\
% 0.819233969869709	0.981844043042175\\
% 0.865544627771694	0.990383180981857\\
% 0.911855285673678	1.00051138400479\\
% 0.958165943575664	1.00116666110939\\
% 1.00447660147765	1.00933417658963\\
% 1.05078725937963	1.02327713063164\\
% 1.09709791728162	1.03405895671487\\
% 1.1434085751836	1.02588494940835\\
% 1.18971923308559	1.03903367414905\\
% 1.23602989098757	1.045321680344\\
% 1.28234054888956	1.04048989613871\\
% 1.32865120679154	1.07829305487271\\
% 1.37496186469353	1.0806197354692\\
% 1.42127252259551	1.07468925575836\\
% 1.4675831804975	1.07525120021827\\
% 1.51389383839948	1.07127376000105\\
% 1.56020449630147	1.07701731877009\\
% 1.60651515420345	1.08372755384067\\
% 1.65282581210544	1.10702969782284\\
% 1.69913647000742	1.1265462618505\\
% 1.7454471279094	1.11964671761876\\
% 1.79175778581139	1.12910478739512\\
% 1.83806844371337	1.12625101323637\\
% 1.88437910161536	1.1279443891836\\
% 1.93068975951734	1.13972729507199\\
% 1.97700041741933	1.18720308561246\\
% 2.02331107532131	1.19549428678842\\
% 2.0696217332233	1.19211630244144\\
% 2.11593239112528	1.18820351597201\\
% 2.16224304902727	1.18946803467231\\
% 2.20855370692925	1.19931279079381\\
% 2.25486436483124	1.20725161945378\\
% 2.30117502273322	1.20144351928871\\
% 2.34748568063521	1.20972361760241\\
% 2.39379633853719	1.24639550411424\\
% 2.44010699643918	1.29770071237523\\
% 2.48641765434116	1.30163150409066\\
% 2.53272831224315	1.303255347462\\
% 2.57903897014513	1.36086866224068\\
% 2.62534962804712	1.34941715116773\\
% 2.6716602859491	1.34552050890205\\
% 2.71797094385109	1.37435385088923\\
% 2.76428160175307	1.28467004070748\\
% 2.81059225965506	1.30321598695837\\
% 2.85690291755704	1.28636887733454\\
% 2.90321357545902	1.37601600420094\\
% 2.94952423336101	1.45689487909069\\
% 2.99583489126299	1.57902806570856\\
% 3.04214554916498	1.55441670393166\\
% 3.08845620706696	1.5197123687683\\
% 3.13476686496895	1.52900976686973\\
% 3.18107752287093	1.53363337049341\\
% 3.22738818077292	1.62932942581715\\
% 3.2736988386749	1.7294295463387\\
% 3.32000949657689	1.68388529367211\\
% 3.36632015447887	1.98364355799848\\
% 3.41263081238086	1.86498083425379\\
% 3.45894147028284	1.71042598231242\\
% 3.50525212818483	2.07630867648239\\
% 3.55156278608681	2.04826170182755\\
% 3.5978734439888	1.87600380756715\\
% 3.64418410189078	1.87850709362784\\
% 3.69049475979277	1.97336876782486\\
% 3.73680541769475	2.2147900111789\\
% 3.78311607559674	1.85577650976018\\
% 3.82942673349872	2.47377536786875\\
% 3.87573739140071	2.8877571869949\\
% 3.92204804930269	2.81120160432625\\
% 3.96835870720468	2.77000688495539\\
% 4.01466936510666	2.6118519912476\\
% 4.06098002300864	2.40177482529855\\
% 4.10729068091063	2.29039443163371\\
% 4.15360133881262	2.48134271902891\\
% 4.1999119967146	2.65881534761359\\
% 4.24622265461658	3.12101471996246\\
% 4.29253331251857	2.71680097467167\\
% 4.33884397042055	3.48114770553597\\
% 4.38515462832254	3.15675026268022\\
% 4.43146528622452	2.00725697820564\\
% 4.47777594412651	3.0849289498584\\
% 4.52408660202849	2.41592129635564\\
% 4.57039725993048	1.83748188511543\\
% 4.61670791783246	1.79450305756125\\
% 4.66301857573445	5.71169015435604\\
% 4.70932923363643	2.45643572006272\\
% 4.75563989153842	5.56148885383769\\
% 4.8019505494404	13.152256402012\\
% 4.84826120734239	32.579667216727\\
% };\nolegendentry{};

% \addplot [color=mycolor6, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor6}, forget plot]
%   table[row sep=crcr]{%
% -4.860551698549	36.8442268992987\\
% -4.80821798771478	8.47848087279959\\
% -4.75588427688057	4.89965917136963\\
% -4.70355056604636	9.07979246038391\\
% -4.65121685521215	10.2754616053657\\
% -4.59888314437793	10.5117984093739\\
% -4.54654943354372	14.3515073562349\\
% -4.49421572270951	9.80287046409075\\
% -4.4418820118753	8.65610809257275\\
% -4.38954830104108	12.7331577230991\\
% -4.33721459020687	12.4744074299288\\
% -4.28488087937266	10.0617432971821\\
% -4.23254716853845	8.70928160836162\\
% -4.18021345770423	9.96292733565959\\
% -4.12787974687002	10.263348127939\\
% -4.07554603603581	9.8018201479313\\
% -4.02321232520159	8.78810883782565\\
% -3.97087861436738	7.66091823589692\\
% -3.91854490353317	6.80283319123618\\
% -3.86621119269896	6.36147075479685\\
% -3.81387748186474	6.64562398872174\\
% -3.76154377103053	7.59048428824442\\
% -3.70921006019632	6.25681607121583\\
% -3.65687634936211	5.14238641630829\\
% -3.60454263852789	5.43904776095896\\
% -3.55220892769368	5.10490226132367\\
% -3.49987521685947	4.91864681543105\\
% -3.44754150602525	4.81776315419258\\
% -3.39520779519104	4.90993719020134\\
% -3.34287408435683	4.86031953720358\\
% -3.29054037352262	4.46471251292512\\
% -3.2382066626884	4.25242884677718\\
% -3.18587295185419	4.0139113325752\\
% -3.13353924101998	3.70698089332672\\
% -3.08120553018577	3.70159097903642\\
% -3.02887181935155	3.64824400660712\\
% -2.97653810851734	3.4311364453864\\
% -2.92420439768313	3.29866151246929\\
% -2.87187068684891	3.21955883229334\\
% -2.8195369760147	3.11008435919531\\
% -2.76720326518049	2.98830916644471\\
% -2.71486955434628	2.91259472347876\\
% -2.66253584351206	2.94084563671981\\
% -2.61020213267785	2.79895140111774\\
% -2.55786842184364	2.60319148358082\\
% -2.50553471100943	2.56879861892368\\
% -2.45320100017521	2.43051334081354\\
% -2.400867289341	2.411048569994\\
% -2.34853357850679	2.32260855943051\\
% -2.29619986767257	2.22904413896699\\
% -2.24386615683836	2.12755262605173\\
% -2.19153244600415	2.038398709321\\
% -2.13919873516994	1.93055012190403\\
% -2.08686502433572	1.91004858084444\\
% -2.03453131350151	1.88343598364016\\
% -1.9821976026673	1.8144335855068\\
% -1.92986389183309	1.75773101497444\\
% -1.87753018099887	1.67392095276024\\
% -1.82519647016466	1.63796037729432\\
% -1.77286275933045	1.59426199440507\\
% -1.72052904849624	1.54092776827423\\
% -1.66819533766202	1.47859012166983\\
% -1.61586162682781	1.43731711800385\\
% -1.5635279159936	1.40166946277916\\
% -1.51119420515938	1.38545109351289\\
% -1.45886049432517	1.34663787055203\\
% -1.40652678349096	1.31464386231598\\
% -1.35419307265675	1.28742827546668\\
% -1.30185936182253	1.23993865365118\\
% -1.24952565098832	1.19523540141589\\
% -1.19719194015411	1.18220181421306\\
% -1.1448582293199	1.15652449940278\\
% -1.09252451848568	1.13095761166966\\
% -1.04019080765147	1.10554134554121\\
% -0.987857096817258	1.07675350639848\\
% -0.935523385983045	1.04151984387888\\
% -0.883189675148832	1.02945499520859\\
% -0.830855964314619	0.999736646610459\\
% -0.778522253480407	0.980057002664146\\
% -0.726188542646194	0.95775126123526\\
% -0.673854831811981	0.937957728753368\\
% -0.621521120977768	0.92430435094948\\
% -0.569187410143556	0.918141004371009\\
% -0.516853699309343	0.920085073861593\\
% -0.46451998847513	0.901326799223285\\
% -0.412186277640918	0.888505198855229\\
% -0.359852566806705	0.872612993492079\\
% -0.307518855972492	0.859860836026456\\
% -0.25518514513828	0.846892225092139\\
% -0.202851434304067	0.842237108741234\\
% -0.150517723469855	0.831585433398412\\
% -0.0981840126356416	0.816497338261942\\
% -0.0458503018014291	0.816488394117565\\
% 0.00648340903278372	0.811803115320559\\
% 0.0588171198669963	0.809461535418938\\
% 0.111150830701209	0.809391538347072\\
% 0.163484541535422	0.808131433595815\\
% 0.215818252369635	0.804375755010618\\
% 0.268151963203847	0.798919408065948\\
% 0.32048567403806	0.79905454014666\\
% 0.372819384872273	0.808936753885087\\
% 0.425153095706485	0.817530063558885\\
% 0.477486806540698	0.817063640071719\\
% 0.529820517374911	0.822358678201337\\
% 0.582154228209123	0.820547836167066\\
% 0.634487939043336	0.83012212447307\\
% 0.686821649877549	0.839875297341288\\
% 0.739155360711761	0.85001079028683\\
% 0.791489071545974	0.854092337702107\\
% 0.843822782380187	0.865254115172337\\
% 0.8961564932144	0.880548534367243\\
% 0.948490204048612	0.895332972340615\\
% 1.00082391488283	0.904525384715808\\
% 1.05315762571704	0.926617190306589\\
% 1.10549133655125	0.94881580293123\\
% 1.15782504738546	0.966491036852275\\
% 1.21015875821968	0.996615675200806\\
% 1.26249246905389	1.00878997471362\\
% 1.3148261798881	1.02658665863475\\
% 1.36715989072231	1.04280257347086\\
% 1.41949360155653	1.05127967582773\\
% 1.47182731239074	1.08666238301969\\
% 1.52416102322495	1.1124578548504\\
% 1.57649473405916	1.15825549014708\\
% 1.62882844489338	1.17454727021053\\
% 1.68116215572759	1.21626250055121\\
% 1.7334958665618	1.21842583173946\\
% 1.78582957739602	1.24082908623761\\
% 1.83816328823023	1.26620456756095\\
% 1.89049699906444	1.29844753217774\\
% 1.94283070989865	1.33999026095487\\
% 1.99516442073287	1.41425362607049\\
% 2.04749813156708	1.42372178633383\\
% 2.09983184240129	1.44509570382268\\
% 2.1521655532355	1.44573854318699\\
% 2.20449926406972	1.51072611926425\\
% 2.25683297490393	1.62117150624588\\
% 2.30916668573814	1.68297441896302\\
% 2.36150039657235	1.68671019099091\\
% 2.41383410740657	1.7388275715152\\
% 2.46616781824078	1.80160027956707\\
% 2.51850152907499	1.83788804260607\\
% 2.57083523990921	1.96574789423207\\
% 2.62316895074342	2.0598218020794\\
% 2.67550266157763	2.2543549404168\\
% 2.72783637241184	2.26999939252157\\
% 2.78017008324606	2.37726871201893\\
% 2.83250379408027	2.48647631036464\\
% 2.88483750491448	2.60265073509375\\
% 2.93717121574869	2.83375928894119\\
% 2.98950492658291	2.81864608933748\\
% 3.04183863741712	2.91940988653642\\
% 3.09417234825133	3.21586227085096\\
% 3.14650605908555	3.25987148463295\\
% 3.19883976991976	3.70330335896661\\
% 3.25117348075397	4.12452229691736\\
% 3.30350719158818	4.3828824854143\\
% 3.3558409024224	4.4530125653765\\
% 3.40817461325661	4.53896665410723\\
% 3.46050832409082	5.0898182449466\\
% 3.51284203492503	5.71434673807983\\
% 3.56517574575925	5.59218683788371\\
% 3.61750945659346	6.12759517255709\\
% 3.66984316742767	6.28225787066654\\
% 3.72217687826189	7.13467836825492\\
% 3.7745105890961	6.55807698409516\\
% 3.82684429993031	6.94678489515757\\
% 3.87917801076452	8.59040500680275\\
% 3.93151172159874	9.44463043303978\\
% 3.98384543243295	10.7420826693741\\
% 4.03617914326716	12.7039661340718\\
% 4.08851285410137	12.2416602139292\\
% 4.14084656493559	14.2045094399911\\
% 4.1931802757698	13.728236236602\\
% 4.24551398660401	16.7248982946336\\
% 4.29784769743822	24.6336432312823\\
% 4.35018140827244	16.516123442427\\
% 4.40251511910665	21.4702039410052\\
% 4.45484882994086	26.2711311830872\\
% 4.50718254077507	26.5487038677022\\
% 4.55951625160929	21.1365095689218\\
% 4.6118499624435	26.3119964012698\\
% 4.66418367327771	30.0460817398154\\
% 4.71651738411193	30.461062058067\\
% 4.76885109494614	40.2932304180422\\
% 4.82118480578035	28.5013271466778\\
% 4.87351851661456	36.6408842558061\\
% 4.92585222744878	47.566040607869\\
% 4.97818593828299	33.7182217380146\\
% 5.0305196491172	67.5598856660683\\
% 5.08285335995141	52.3987910095208\\
% 5.13518707078563	143.623133167871\\
% 5.18752078161984	485.62183083435\\
% 5.23985449245405	206.971306444473\\
% 5.29218820328827	39.2131093034498\\
% 5.34452191412248	64.263084317461\\
% 5.39685562495669	51.5167374226461\\
% 5.4491893357909	142.339205974089\\
% 5.50152304662512	258.7478730347\\
% 5.55385675745933	1074.0379156008\\
% };
% \nolegendentry{};

% \addplot [color=mycolor7, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor7}, forget plot]
%   table[row sep=crcr]{%
% -3.87822575924531	0.696019913646553\\
% -3.83214113154068	0.26814916144231\\
% -3.78605650383605	0.273657976016474\\
% -3.73997187613142	0.344896274060428\\
% -3.69388724842679	0.35928536344527\\
% -3.64780262072216	0.20734211526664\\
% -3.60171799301753	0.322829108603373\\
% -3.55563336531291	0.432697288442152\\
% -3.50954873760828	0.51097805546516\\
% -3.46346410990365	0.492268369480417\\
% -3.41737948219902	0.552480328250371\\
% -3.37129485449439	0.617794975033102\\
% -3.32521022678976	0.580159377674328\\
% -3.27912559908513	0.538735374240201\\
% -3.2330409713805	0.393299367275304\\
% -3.18695634367587	0.533507019785443\\
% -3.14087171597124	0.634933226369558\\
% -3.09478708826661	0.67903367654058\\
% -3.04870246056198	0.685146236828986\\
% -3.00261783285736	0.741057077421685\\
% -2.95653320515273	0.827237197796896\\
% -2.9104485774481	0.824728504539346\\
% -2.86436394974347	0.837960568144341\\
% -2.81827932203884	0.859922907569803\\
% -2.77219469433421	0.895422000098484\\
% -2.72611006662958	0.958832775908504\\
% -2.68002543892495	0.985946560671348\\
% -2.63394081122032	0.934401857613637\\
% -2.58785618351569	1.00567430417257\\
% -2.54177155581106	1.05846026472658\\
% -2.49568692810644	1.01336672122206\\
% -2.44960230040181	1.05212821377208\\
% -2.40351767269718	1.08619303108356\\
% -2.35743304499255	1.12127645848185\\
% -2.31134841728792	1.06257230434169\\
% -2.26526378958329	1.05729448512101\\
% -2.21917916187866	1.12310725828602\\
% -2.17309453417403	1.15582527888125\\
% -2.1270099064694	1.16545486145154\\
% -2.08092527876477	1.15851702098647\\
% -2.03484065106015	1.18728503320253\\
% -1.98875602335552	1.17826669463442\\
% -1.94267139565089	1.17049260692023\\
% -1.89658676794626	1.18797661971181\\
% -1.85050214024163	1.18089395190144\\
% -1.804417512537	1.2034729350307\\
% -1.75833288483237	1.20200874785309\\
% -1.71224825712774	1.18509792942233\\
% -1.66616362942311	1.17430947504401\\
% -1.62007900171848	1.15454534136289\\
% -1.57399437401385	1.15581669258939\\
% -1.52790974630923	1.15759705263982\\
% -1.4818251186046	1.15495467268407\\
% -1.43574049089997	1.1441097959327\\
% -1.38965586319534	1.13573917585099\\
% -1.34357123549071	1.124972297107\\
% -1.29748660778608	1.1141372159807\\
% -1.25140198008145	1.12413397390341\\
% -1.20531735237682	1.10382791298482\\
% -1.15923272467219	1.08025338792723\\
% -1.11314809696756	1.07767936742565\\
% -1.06706346926293	1.07981549570928\\
% -1.02097884155831	1.07598203406794\\
% -0.974894213853676	1.07185183011182\\
% -0.928809586149047	1.06179921904876\\
% -0.882724958444418	1.04654243172612\\
% -0.836640330739789	1.05465990812585\\
% -0.79055570303516	1.05441632222847\\
% -0.744471075330531	1.05481487621712\\
% -0.698386447625902	1.03435945734771\\
% -0.652301819921273	1.02675088388348\\
% -0.606217192216644	1.0190191951827\\
% -0.560132564512015	1.01894326457699\\
% -0.514047936807386	1.01934351925305\\
% -0.467963309102756	1.00993275684737\\
% -0.421878681398128	0.998113727137011\\
% -0.375794053693498	0.982669872858878\\
% -0.329709425988869	0.975356219230589\\
% -0.28362479828424	0.972088381751423\\
% -0.237540170579611	0.967238855741769\\
% -0.191455542874982	0.96619274082058\\
% -0.145370915170353	0.962139678227135\\
% -0.0992862874657242	0.956068897201557\\
% -0.0532016597610948	0.950988977556264\\
% -0.0071170320564658	0.935265745784063\\
% 0.0389675956481632	0.930606448963925\\
% 0.0850522233527922	0.930496583824567\\
% 0.131136851057422	0.93065977814688\\
% 0.17722147876205	0.939312456781055\\
% 0.22330610646668	0.932930414046404\\
% 0.269390734171308	0.933497078833484\\
% 0.315475361875938	0.925398211497895\\
% 0.361559989580567	0.910560321587887\\
% 0.407644617285196	0.91213135759527\\
% 0.453729244989825	0.916183892264755\\
% 0.499813872694454	0.908071646373362\\
% 0.545898500399083	0.900508450785953\\
% 0.591983128103712	0.910328487476417\\
% 0.638067755808341	0.89371920669227\\
% 0.68415238351297	0.901266804985372\\
% 0.730237011217599	0.919270929793132\\
% 0.776321638922228	0.907089056058057\\
% 0.822406266626858	0.907612092188734\\
% 0.868490894331487	0.913494547490822\\
% 0.914575522036116	0.919784681018057\\
% 0.960660149740745	0.912866225803555\\
% 1.00674477744537	0.914095522997676\\
% 1.05282940515	0.919999781585173\\
% 1.09891403285463	0.917408596362517\\
% 1.14499866055926	0.925344216381554\\
% 1.19108328826389	0.944711080799182\\
% 1.23716791596852	0.946123064835705\\
% 1.28325254367315	0.953896521254892\\
% 1.32933717137778	0.956972482761784\\
% 1.37542179908241	0.973542197101693\\
% 1.42150642678704	0.974807418846631\\
% 1.46759105449167	0.98851414727105\\
% 1.51367568219629	1.00710572264877\\
% 1.55976030990092	1.01396935536979\\
% 1.60584493760555	1.01877672296313\\
% 1.65192956531018	1.0209952231219\\
% 1.69801419301481	1.03856402560746\\
% 1.74409882071944	1.06669943086646\\
% 1.79018344842407	1.09200279722963\\
% 1.8362680761287	1.11763714592198\\
% 1.88235270383333	1.12965991422109\\
% 1.92843733153796	1.14667328834216\\
% 1.97452195924258	1.17664776600944\\
% 2.02060658694721	1.20640122014328\\
% 2.06669121465184	1.2015103418157\\
% 2.11277584235647	1.23116742604364\\
% 2.1588604700611	1.27742277029678\\
% 2.20494509776573	1.26225394518923\\
% 2.25102972547036	1.29763182157264\\
% 2.29711435317499	1.3742046776993\\
% 2.34319898087962	1.47060177753164\\
% 2.38928360858425	1.50683477806436\\
% 2.43536823628887	1.51998459413917\\
% 2.4814528639935	1.50509186989373\\
% 2.52753749169813	1.55035054528094\\
% 2.57362211940276	1.61505701777669\\
% 2.61970674710739	1.61273991945866\\
% 2.66579137481202	1.69711611868724\\
% 2.71187600251665	1.75969552473415\\
% 2.75796063022128	1.79891563303844\\
% 2.80404525792591	1.90743655665455\\
% 2.85012988563054	1.92169830831824\\
% 2.89621451333517	2.01445448647949\\
% 2.9422991410398	2.18204707492333\\
% 2.98838376874442	2.22130987030273\\
% 3.03446839644905	2.29552405582202\\
% 3.08055302415368	2.45021020227234\\
% 3.12663765185831	2.74513018129252\\
% 3.17272227956294	2.83624408325293\\
% 3.21880690726757	2.83349007708311\\
% 3.2648915349722	2.94975450260418\\
% 3.31097616267683	3.46940875109552\\
% 3.35706079038146	3.38413879322846\\
% 3.40314541808609	3.7370288197837\\
% 3.44923004579072	3.84988042056492\\
% 3.49531467349534	3.70012380491524\\
% 3.54139930119997	4.09757736205377\\
% 3.5874839289046	4.45425914681825\\
% 3.63356855660923	4.66902439629355\\
% 3.67965318431386	4.8793908421996\\
% 3.72573781201849	5.62771291315921\\
% 3.77182243972312	6.16427352425432\\
% 3.81790706742775	6.27112338496815\\
% 3.86399169513238	6.59413438482178\\
% 3.91007632283701	6.15262402656134\\
% 3.95616095054163	6.48539161350118\\
% 4.00224557824626	8.64890322506782\\
% 4.04833020595089	9.24547236536868\\
% 4.09441483365552	8.10127929595257\\
% 4.14049946136015	7.55559450516723\\
% 4.18658408906478	7.14339507624031\\
% 4.23266871676941	6.76642139544883\\
% 4.27875334447404	8.37237846052189\\
% 4.32483797217867	11.3553070879562\\
% 4.3709225998833	12.150946949422\\
% 4.41700722758792	17.4455263578055\\
% 4.46309185529255	21.5195406119126\\
% 4.50917648299718	24.4132303289235\\
% 4.55526111070181	19.4678854745344\\
% 4.60134573840644	19.8351032172898\\
% 4.64743036611107	19.6921063611376\\
% 4.6935149938157	20.5767402439498\\
% 4.73959962152033	17.4077885304139\\
% 4.78568424922496	28.1841038268499\\
% 4.83176887692959	17.4339592946739\\
% 4.87785350463422	9.87942036672192\\
% 4.92393813233885	28.0140521880974\\
% 4.97002276004347	10.6965556275634\\
% 5.0161073877481	28.852082751178\\
% 5.06219201545273	65.2514053537038\\
% 5.10827664315736	65.4672558354785\\
% 5.15436127086199	123.269276486748\\
% 5.20044589856662	29.3610359514365\\
% 5.24653052627125	75.2839601167235\\
% 5.29261515397588	362.1765561849\\
% };
% \nolegendentry{};

% \addplot [color=mycolor8, line width=1.0pt, draw = none, mark=o, mark size = 1pt,mark options={solid, mycolor8}, forget plot]
%   table[row sep=crcr]{%
% -4.12658275808832	1.86653009274671\\
% -4.07424631366351	1.17367265357447\\
% -4.02190986923869	0.736938882927558\\
% -3.96957342481388	0.737742357635525\\
% -3.91723698038906	0.828222687455887\\
% -3.86490053596424	0.717963029917197\\
% -3.81256409153943	0.75580038454552\\
% -3.76022764711461	1.10847286769618\\
% -3.7078912026898	0.922883732332492\\
% -3.65555475826498	0.951134176439066\\
% -3.60321831384017	0.948025429956758\\
% -3.55088186941535	0.950926127212651\\
% -3.49854542499053	1.21827161028606\\
% -3.44620898056572	1.06395222340271\\
% -3.3938725361409	1.01608324534551\\
% -3.34153609171609	1.11975208385073\\
% -3.28919964729127	1.1169032356437\\
% -3.23686320286645	1.05895405219506\\
% -3.18452675844164	1.0954613369049\\
% -3.13219031401682	1.10284096979236\\
% -3.07985386959201	1.11614095960627\\
% -3.02751742516719	1.23738419070727\\
% -2.97518098074237	1.09711475946206\\
% -2.92284453631756	1.04743425360903\\
% -2.87050809189274	1.13112906291152\\
% -2.81817164746793	1.16667065511952\\
% -2.76583520304311	1.19311267145174\\
% -2.71349875861829	1.24346574086472\\
% -2.66116231419348	1.25996315327795\\
% -2.60882586976866	1.1694646009631\\
% -2.55648942534385	1.18660044858954\\
% -2.50415298091903	1.19438232862994\\
% -2.45181653649422	1.25445493826201\\
% -2.3994800920694	1.25200286659255\\
% -2.34714364764458	1.22782372983572\\
% -2.29480720321977	1.22798024708691\\
% -2.24247075879495	1.27497454053518\\
% -2.19013431437014	1.29802012998389\\
% -2.13779786994532	1.28759777980533\\
% -2.0854614255205	1.27687801566664\\
% -2.03312498109569	1.2683961415954\\
% -1.98078853667087	1.27535760861798\\
% -1.92845209224606	1.25815557288713\\
% -1.87611564782124	1.25101658842851\\
% -1.82377920339642	1.27906358157061\\
% -1.77144275897161	1.27146814062373\\
% -1.71910631454679	1.23831607610797\\
% -1.66676987012198	1.23161383553524\\
% -1.61443342569716	1.2448294268853\\
% -1.56209698127234	1.23007222615715\\
% -1.50976053684753	1.21502519188496\\
% -1.45742409242271	1.17893532547954\\
% -1.4050876479979	1.17338759797704\\
% -1.35275120357308	1.17823437659107\\
% -1.30041475914826	1.1647675553123\\
% -1.24807831472345	1.1634539996735\\
% -1.19574187029863	1.15496297180976\\
% -1.14340542587382	1.1264955830972\\
% -1.091068981449	1.11867907547357\\
% -1.03873253702419	1.10712979597157\\
% -0.98639609259937	1.09689335886828\\
% -0.934059648174554	1.08666359070589\\
% -0.881723203749738	1.06838512121701\\
% -0.829386759324922	1.05875261857876\\
% -0.777050314900106	1.05245276840722\\
% -0.72471387047529	1.0476201625097\\
% -0.672377426050474	1.02821395611625\\
% -0.620040981625658	1.01045228957717\\
% -0.567704537200842	1.01034049957297\\
% -0.515368092776026	0.995184640266654\\
% -0.46303164835121	0.98606988035647\\
% -0.410695203926394	0.981245593523472\\
% -0.358358759501578	0.97518477903536\\
% -0.306022315076762	0.981074110534321\\
% -0.253685870651947	0.976365261361665\\
% -0.201349426227131	0.963624745753158\\
% -0.149012981802315	0.967005530586832\\
% -0.096676537377499	0.966064576319394\\
% -0.0443400929526828	0.958941547167395\\
% 0.00799635147213285	0.947667397741958\\
% 0.060332795896949	0.943895857483646\\
% 0.112669240321765	0.941586831766788\\
% 0.165005684746581	0.936068798454443\\
% 0.217342129171397	0.932108706981639\\
% 0.269678573596213	0.925142938341679\\
% 0.322015018021028	0.926430482702527\\
% 0.374351462445844	0.930001872458317\\
% 0.42668790687066	0.92182345662704\\
% 0.479024351295476	0.926567750394652\\
% 0.531360795720292	0.936442986409338\\
% 0.583697240145108	0.936977470425163\\
% 0.636033684569924	0.929045012642367\\
% 0.68837012899474	0.917593444757643\\
% 0.740706573419556	0.916824393630192\\
% 0.793043017844372	0.924748554605061\\
% 0.845379462269187	0.932012285686043\\
% 0.897715906694003	0.943096269625904\\
% 0.950052351118819	0.940828141479564\\
% 1.00238879554364	0.940113517174892\\
% 1.05472523996845	0.945745494128762\\
% 1.10706168439327	0.94350241759922\\
% 1.15939812881808	0.955768260870435\\
% 1.2117345732429	0.957865058577545\\
% 1.26407101766771	0.946549770914806\\
% 1.31640746209253	0.962856835902157\\
% 1.36874390651735	0.963127688495944\\
% 1.42108035094216	0.963089914113794\\
% 1.47341679536698	0.973265240658849\\
% 1.52575323979179	0.982709587164739\\
% 1.57808968421661	0.97701202357858\\
% 1.63042612864143	0.98816059641381\\
% 1.68276257306624	0.993728737232458\\
% 1.73509901749106	0.990775162857251\\
% 1.78743546191587	0.991882101521809\\
% 1.83977190634069	1.02868051655306\\
% 1.89210835076551	1.05126295976836\\
% 1.94444479519032	1.05117085639849\\
% 1.99678123961514	1.03695617696604\\
% 2.04911768403995	1.08207533607931\\
% 2.10145412846477	1.11605453324945\\
% 2.15379057288959	1.12065432707301\\
% 2.2061270173144	1.13254941689556\\
% 2.25846346173922	1.17037173266064\\
% 2.31079990616403	1.15906943664859\\
% 2.36313635058885	1.18440314378323\\
% 2.41547279501366	1.1980058074759\\
% 2.46780923943848	1.2477394148523\\
% 2.5201456838633	1.29022666039079\\
% 2.57248212828811	1.34996842127184\\
% 2.62481857271293	1.40027416521069\\
% 2.67715501713774	1.46340758695456\\
% 2.72949146156256	1.50602934035001\\
% 2.78182790598738	1.49007375448317\\
% 2.83416435041219	1.57005223919686\\
% 2.88650079483701	1.48217325891633\\
% 2.93883723926182	1.63287927853914\\
% 2.99117368368664	1.79023041524365\\
% 3.04351012811146	1.90616652104669\\
% 3.09584657253627	1.91005246015996\\
% 3.14818301696109	1.98778630211482\\
% 3.2005194613859	2.26859626158591\\
% 3.25285590581072	2.33155901765428\\
% 3.30519235023554	2.41343025810636\\
% 3.35752879466035	2.46944240703057\\
% 3.40986523908517	2.6349637510805\\
% 3.46220168350998	2.88656447001968\\
% 3.5145381279348	3.51444021709764\\
% 3.56687457235962	3.58442274949724\\
% 3.61921101678443	3.82554519566429\\
% 3.67154746120925	4.52448807492525\\
% 3.72388390563406	4.78505670403142\\
% 3.77622035005888	5.4444005845398\\
% 3.8285567944837	5.6256267858755\\
% 3.88089323890851	5.99657377321746\\
% 3.93322968333333	7.54981907852313\\
% 3.98556612775814	9.01510143894633\\
% 4.03790257218296	8.64189250301472\\
% 4.09023901660777	8.59579242261761\\
% 4.14257546103259	10.5132320155968\\
% 4.19491190545741	9.73260041114376\\
% 4.24724834988222	11.4372490426908\\
% 4.29958479430704	11.4561345559531\\
% 4.35192123873185	15.4968094766621\\
% 4.40425768315667	21.0190571246395\\
% 4.45659412758149	21.2362247196199\\
% 4.5089305720063	18.7143595653908\\
% 4.56126701643112	30.3571241131285\\
% 4.61360346085593	28.4498439886443\\
% 4.66593990528075	41.738172486483\\
% 4.71827634970556	45.8416843248386\\
% 4.77061279413038	47.0140300751288\\
% 4.8229492385552	45.0343741053297\\
% 4.87528568298001	62.1505529588404\\
% 4.92762212740483	81.7297515137223\\
% 4.97995857182965	72.8453105084206\\
% 5.03229501625446	96.4967399883942\\
% 5.08463146067928	152.141384296929\\
% 5.13696790510409	116.467125197379\\
% 5.18930434952891	156.977319972954\\
% 5.24164079395372	88.9737495678392\\
% 5.29397723837854	104.337722117799\\
% 5.34631368280336	193.041405821393\\
% 5.39865012722817	135.286163618579\\
% 5.45098657165299	69.53449767548\\
% 5.5033230160778	239.185878485269\\
% 5.55565946050262	273.695127453809\\
% 5.60799590492744	274.791500085989\\
% 5.66033234935225	1167.83271040484\\
% 5.71266879377707	1397.15890283453\\
% 5.76500523820188	294.056277035293\\
% 5.8173416826267	0\\
% 5.86967812705152	853.213119489288\\
% 5.92201457147633	3421.71871535863\\
% 5.97435101590115	1777.81102680032\\
% 6.02668746032596	3707.99966779848\\
% 6.07902390475078	2569.843499906\\
% 6.1313603491756	6598.07908124202\\
% 6.18369679360041	1645.24559259497\\
% 6.23603323802523	17271.887554895\\
% 6.28836968245004	83091.7069684693\\
% };
% \nolegendentry{};

% \addplot [color=black, dashed, line width = 0.5pt]
%   table[row sep=crcr]{%
% -6	1\\
% 6	1\\
% };
% \addlegendentry{\footnotesize Gaussian};

% % \addplot[area legend, draw=black, fill=black, fill opacity=0.01]
% % table[row sep=crcr] {%
% % x	y\\
% % -6	0.909090909090\\
% % 6	0.909090909090\\
% % 6	1.1\\
% % -6	1.1\\
% % }--cycle;
%  \addplot[fill=black, fill opacity = 0.1, draw = none,area legend] coordinates {(-6,0.9090909090) (6,0.9090909090) (6,1.1) (-6,1.1)};
% \addlegendentry{\footnotesize $\pm10\%$};

% \end{axis}

